The not so simple globular cluster $\omega$ Cen. I. Spatial distribution of the multiple stellar populations

We present a multi-band photometric catalog of $\approx$ 1.7 million cluster members for a field of view of $\approx$ 2x2 degree across $\omega$ Cen. Photometry is based on images collected with the Dark Energy Camera on the 4m Blanco telescope and the Advanced Camera for Surveys on the Hubble Space Telescope. The unprecedented photometric accuracy and field coverage allowed us for the first time to investigate the spatial distribution of $\omega$ Cen multiple populations from the core to the tidal radius, confirming its very complex structure. We found that the frequency of blue main-sequence stars is increasing compared to red main-sequence stars starting from a distance of $\approx$ 25' from the cluster center. Blue main-sequence stars also show a clumpy spatial distribution, with an excess in the North-East quadrant of the cluster pointing towards the direction of the Galactic center. Stars belonging to the reddest and faintest red-giant branch also show a more extended spatial distribution in the outskirts of $\omega$ Cen, a region never explored before. Both these stellar sub-populations, according to spectroscopic measurements, are more metal-rich compared to the cluster main stellar population. These findings, once confirmed, make $\omega$ Cen the only stellar system currently known where metal-rich stars have a more extended spatial distribution compared to metal-poor stars. Kinematic and chemical abundance measurements are now needed for stars in the external regions of $\omega$ Cen to better characterize the properties of these sub-populations.

==> calamida <==
@ARTICLE{ho2015,
   author = {{Ho}, N. and {Geha}, M. and {Tollerud}, E.~J. and {Zinn}, R. and 
	{Guhathakurta}, P. and {Vargas}, L.~C.},
    title = "{Metallicity Evolution of the Six Most Luminous M31 Dwarf Satellites}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1405.4424},
 keywords = {galaxies: abundances, galaxies: dwarf, galaxies: individual: M32 NGC 205 NGC 185 NGC 147 And VII And II, Local Group},
     year = 2015,
    month = jan,
   volume = 798,
      eid = {77},
    pages = {77},
      doi = {10.1088/0004-637X/798/2/77},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...798...77H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{marino2012,
   author = {{Marino}, A.~F. and {Milone}, A.~P. and {Piotto}, G. and {Cassisi}, S. and 
	{D'Antona}, F. and {Anderson}, J. and {Aparicio}, A. and {Bedin}, L.~R. and 
	{Renzini}, A. and {Villanova}, S.},
    title = "{The C+N+O Abundance of {$\omega$} Centauri Giant Stars: Implications for the Chemical-enrichment Scenario and the Relative Ages of Different Stellar Populations}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1111.1891},
 primaryClass = "astro-ph.SR",
 keywords = {globular clusters: individual: NGC 5139, stars: abundances, stars: Population II},
     year = 2012,
    month = feb,
   volume = 746,
      eid = {14},
    pages = {14},
      doi = {10.1088/0004-637X/746/1/14},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...746...14M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{marino2011,
   author = {{Marino}, A.~F. and {Milone}, A.~P. and {Piotto}, G. and {Villanova}, S. and 
	{Gratton}, R. and {D'Antona}, F. and {Anderson}, J. and {Bedin}, L.~R. and 
	{Bellini}, A. and {Cassisi}, S. and {Geisler}, D. and {Renzini}, A. and 
	{Zoccali}, M.},
    title = "{Sodium-Oxygen Anticorrelation and Neutron-capture Elements in Omega Centauri Stellar Populations}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1102.1653},
 primaryClass = "astro-ph.SR",
 keywords = {globular clusters: individual: NGC 5139, stars: abundances, stars: Population II},
     year = 2011,
    month = apr,
   volume = 731,
      eid = {64},
    pages = {64},
      doi = {10.1088/0004-637X/731/1/64},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...731...64M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{gratton2011,
   author = {{Gratton}, R.~G. and {Johnson}, C.~I. and {Lucatello}, S. and 
	{D'Orazi}, V. and {Pilachowski}, C.},
    title = "{Multiple populations in {$\omega$} Centauri: a cluster analysis of spectroscopic data}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1105.5544},
 keywords = {stars: abundances, stars: evolution, stars: Population II, globular clusters: individual: omega Centauri},
     year = 2011,
    month = oct,
   volume = 534,
      eid = {A72},
    pages = {A72},
      doi = {10.1051/0004-6361/201117093},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...534A..72G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{ferraro2002,
   author = {{Ferraro}, F.~R. and {Bellazzini}, M. and {Pancino}, E.},
    title = "{Discovery of an Accreted Stellar System within the Globular Cluster {$\omega$} Centauri}",
  journal = {\apjl},
   eprint = {astro-ph/0206145},
 keywords = {Galaxy: Globular Clusters: Individual: Name: {$\omega$} Centauri, Stars: Kinematics, Stars: Population II},
     year = 2002,
    month = jul,
   volume = 573,
    pages = {L95-L99},
      doi = {10.1086/342087},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...573L..95F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{schlafly2011,
   author = {{Schlafly}, E.~F. and {Finkbeiner}, D.~P.},
    title = "{Measuring Reddening with Sloan Digital Sky Survey Stellar Spectra and Recalibrating SFD}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1012.4804},
 primaryClass = "astro-ph.GA",
 keywords = {dust, extinction, Galaxy: stellar content, ISM: clouds},
     year = 2011,
    month = aug,
   volume = 737,
      eid = {103},
    pages = {103},
      doi = {10.1088/0004-637X/737/2/103},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...737..103S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{ferraro2004,
   author = {{Ferraro}, F.~R. and {Sollima}, A. and {Pancino}, E. and {Bellazzini}, M. and 
	{Straniero}, O. and {Origlia}, L. and {Cool}, A.~M.},
    title = "{The Discovery of an Anomalous Subgiant Branch in the Color-Magnitude Diagram of {$\omega$} Centauri}",
  journal = {\apjl},
   eprint = {astro-ph/0401540},
 keywords = {Galaxy: Globular Clusters: Individual: Name: {$\omega$} Centauri, Stars: Evolution, Stars: Population II},
     year = 2004,
    month = mar,
   volume = 603,
    pages = {L81-L84},
      doi = {10.1086/383149},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...603L..81F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{leon2000,
   author = {{Leon}, S. and {Meylan}, G. and {Combes}, F.},
    title = "{Tidal tails around 20 Galactic globular clusters. Observational evidence for gravitational disk/bulge shocking}",
  journal = {\aap},
   eprint = {astro-ph/0006100},
 keywords = {TECHNIQUES: IMAGE PROCESSING, ISM: DUST, EXTINCTION, GALAXY: GLOBULAR CLUSTERS: GENERAL, GALAXY: STRUCTURE, COSMOLOGY: LARGE-SCALE STRUCTURE OF UNIVERSE},
     year = 2000,
    month = jul,
   volume = 359,
    pages = {907-931},
   adsurl = {http://adsabs.harvard.edu/abs/2000A%26A...359..907L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{dauphole1996,
   author = {{Dauphole}, B. and {Geffert}, M. and {Colin}, J. and {Ducourant}, C. and 
	{Odenkirchen}, M. and {Tucholke}, H.-J.},
    title = "{The kinematics of globular clusters, apocentric distances and a halo metallicity gradient.}",
  journal = {\aap},
 keywords = {GLOBULAR CLUSTERS: GENERAL, GALAXY: KINEMATICS AND DYNAMICS, GALAXY: HALO, GALAXY: EVOLUTION, GALAXY: ABUNDANCES},
     year = 1996,
    month = sep,
   volume = 313,
    pages = {119-128},
   adsurl = {http://adsabs.harvard.edu/abs/1996A%26A...313..119D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{fabrizio2015,
   author = {{Fabrizio}, M. and {Nonino}, M. and {Bono}, G. and {Primas}, F. and 
	{Th{\'e}venin}, F. and {Stetson}, P.~B. and {Cassisi}, S. and 
	{Buonanno}, R. and {Coppola}, G. and {da Silva}, R.~O. and {Dall'Ora}, M. and 
	{Ferraro}, I. and {Genovali}, K. and {Gilmozzi}, R. and {Iannicola}, G. and 
	{Marconi}, M. and {Monelli}, M. and {Romaniello}, M. and {Walker}, A.~R.
	},
    title = "{The Carina Project. VIII. The {$\alpha$}-element abundances}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1505.06597},
 keywords = {galaxies: dwarf, galaxies: stellar content, stars: fundamental parameters, galaxies: individual: Carina, stars: abundances},
     year = 2015,
    month = aug,
   volume = 580,
      eid = {A18},
    pages = {A18},
      doi = {10.1051/0004-6361/201525753},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...580A..18F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{bono2010,
   author = {{Bono}, G. and {Stetson}, P.~B. and {Walker}, A.~R. and {Monelli}, M. and 
	{Fabrizio}, M. and {Pietrinferni}, A. and {Brocato}, E. and 
	{Buonanno}, R. and {Caputo}, F. and {Cassisi}, S. and {Castellani}, M. and 
	{Cignoni}, M. and {Corsi}, C.~E. and {Dall'Ora}, M. and {Degl'Innocenti}, S. and 
	{Fran{\c c}ois}, P. and {Ferraro}, I. and {Iannicola}, G. and 
	{Nonino}, M. and {Prada Moroni}, P.~G. and {Pulone}, L. and 
	{Smith}, H.~A. and {Thevenin}, F.},
    title = "{On the Stellar Content of the Carina Dwarf Spheroidal Galaxy}",
  journal = {\pasp},
archivePrefix = "arXiv",
   eprint = {1004.2559},
     year = 2010,
    month = jun,
   volume = 122,
    pages = {651-661},
      doi = {10.1086/653590},
   adsurl = {http://adsabs.harvard.edu/abs/2010PASP..122..651B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{schechter1993,
   author = {{Schechter}, P.~L. and {Mateo}, M. and {Saha}, A.},
    title = "{DOPHOT, a CCD photometry program: Description and tests}",
  journal = {\pasp},
 keywords = {Astronomical Photometry, Charge Coupled Devices, Computer Programs, Computerized Simulation, Data Reduction, Image Processing, Point Spread Functions, Comparison, Globular Clusters, Stellar Color, Stellar Magnitude},
     year = 1993,
    month = nov,
   volume = 105,
    pages = {1342-1353},
      doi = {10.1086/133316},
   adsurl = {http://adsabs.harvard.edu/abs/1993PASP..105.1342S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{sollima2009,
   author = {{Sollima}, A. and {Bellazzini}, M. and {Smart}, R.~L. and {Correnti}, M. and 
	{Pancino}, E. and {Ferraro}, F.~R. and {Romano}, D.},
    title = "{The non-peculiar velocity dispersion profile of the stellar system {$\omega$} Centauri}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0904.0571},
 primaryClass = "astro-ph.SR",
 keywords = {techniques: radial velocities , stars: kinematics , stars: Population II , globular clusters: individual: {$\omega$} Centauri},
     year = 2009,
    month = jul,
   volume = 396,
    pages = {2183-2193},
      doi = {10.1111/j.1365-2966.2009.14864.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.396.2183S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{mayor1997,
   author = {{Mayor}, M. and {Meylan}, G. and {Udry}, S. and {Duquennoy}, A. and 
	{Andersen}, J. and {Nordstrom}, B. and {Imbert}, M. and {Maurice}, E. and 
	{Prevot}, L. and {Ardeberg}, A. and {Lindgren}, H.},
    title = "{Radial velocities of southern stars obtained with the photoelectric scanner coravel, VIII. Observations of 471 giant stars in omega centauri.}",
  journal = {\aj},
 keywords = {GLOBULAR CLUSTERS: INDIVIDUAL: OMEGA CENTAURI, GALAXY: KINEMATICS AND DYNAMICS},
     year = 1997,
    month = sep,
   volume = 114,
    pages = {1087-1097},
      doi = {10.1086/118539},
   adsurl = {http://adsabs.harvard.edu/abs/1997AJ....114.1087M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{norris1997,
   author = {{Norris}, J.~E. and {Freeman}, K.~C. and {Mayor}, M. and {Seitzer}, P.
	},
    title = "{The Giant Branch of {$\omega$} Centauri: The Dependence of Kinematics on Abundance}",
  journal = {\apjl},
 keywords = {GALAXY: GLOBULAR CLUSTERS: INDIVIDUAL NAME: OMEGA CENTAURI, STARS: ABUNDANCES, STARS: KINEMATICS, STARS: POPULATION II, Galaxy: Globular Clusters: Individual: Name: {$\omega$} Centauri, Stars: Abundances, Stars: Kinematics, Stars: Population II},
     year = 1997,
    month = oct,
   volume = 487,
    pages = {L187-L190},
      doi = {10.1086/310895},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...487L.187N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{delpino2013,
   author = {{del Pino}, A. and {Hidalgo}, S.~L. and {Aparicio}, A. and {Gallart}, C. and 
	{Carrera}, R. and {Monelli}, M. and {Buonanno}, R. and {Marconi}, G.
	},
    title = "{Spatial dependence of the star formation history in the central regions of the Fornax dwarf spheroidal galaxy}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1305.2166},
 keywords = {galaxies: dwarf, galaxies: evolution, Local Group, early Universe},
     year = 2013,
    month = aug,
   volume = 433,
    pages = {1505-1516},
      doi = {10.1093/mnras/stt833},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.433.1505D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{martinez2016,
   author = {{Mart{\'{\i}}nez-V{\'a}zquez}, C.~E. and {Monelli}, M. and {Gallart}, C. and 
	{Bono}, G. and {Bernard}, E.~J. and {Stetson}, P.~B. and {Ferraro}, I. and 
	{Walker}, A.~R. and {Dall'Ora}, M. and {Fiorentino}, G. and 
	{Iannicola}, G.},
    title = "{Probing the early chemical evolution of the Sculptor dSph with purely old stellar tracers}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1605.02768},
 keywords = {stars: variables: RR Lyrae, galaxies: evolution, galaxies: individual: Sculptor dSph, Local Group, galaxies: stellar content},
     year = 2016,
    month = sep,
   volume = 461,
    pages = {L41-L45},
      doi = {10.1093/mnrasl/slw093},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.461L..41M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{monelli2003,
   author = {{Monelli}, M. and {Pulone}, L. and {Corsi}, C.~E. and {Castellani}, M. and 
	{Bono}, G. and {Walker}, A.~R. and {Brocato}, E. and {Buonanno}, R. and 
	{Caputo}, F. and {Castellani}, V. and {Dall'Ora}, M. and {Marconi}, M. and 
	{Nonino}, M. and {Ripepi}, V. and {Smith}, H.~A.},
    title = "{The Carina Project. II. Stellar Populations}",
  journal = {\aj},
   eprint = {astro-ph/0303493},
 keywords = {Galaxies: Formation, Galaxies: Individual: Name: Carina, Galaxies: Structure, Galaxies: Local Group, Stars: Evolution},
     year = 2003,
    month = jul,
   volume = 126,
    pages = {218-236},
      doi = {10.1086/375457},
   adsurl = {http://adsabs.harvard.edu/abs/2003AJ....126..218M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{ferraro2016,
   author = {{Ferraro}, F.~R. and {Massari}, D. and {Dalessandro}, E. and 
	{Lanzoni}, B. and {Origlia}, L. and {Rich}, R.~M. and {Mucciarelli}, A.
	},
    title = "{The Age of the Young Bulge-like Population in the Stellar System Terzan 5: Linking the Galactic Bulge to the High-z Universe}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1609.01515},
 keywords = {Galaxy: bulge, globular clusters: Individual: Terzan 5, techniques: photometric },
     year = 2016,
    month = sep,
   volume = 828,
      eid = {75},
    pages = {75},
      doi = {10.3847/0004-637X/828/2/75},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...828...75F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{cannonstobie1973,
   author = {{Cannon}, R.~D. and {Stobie}, R.~S.},
    title = "{Photometry of southern globular clusters I. Bright stars in omega Centauri}",
  journal = {\mnras},
     year = 1973,
   volume = 162,
    pages = {207},
      doi = {10.1093/mnras/162.3.207},
   adsurl = {http://adsabs.harvard.edu/abs/1973MNRAS.162..207C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{mayor1996,
   author = {{Mayor}, M. and {Duquennoy}, A. and {Udry}, S. and {Andersen}, J. and 
	{Nordstrom}, B.},
    title = "{Primordial Binaries in the Globular Cluster {$\omega$} Centauri}",
booktitle = {The Origins, Evolution, and Destinies of Binary Stars in Clusters},
     year = 1996,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 90,
   editor = {{Milone}, E.~F. and {Mermilliod}, J.-C.},
    pages = {190},
   adsurl = {http://adsabs.harvard.edu/abs/1996ASPC...90..190M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{sollima2007c,
   author = {{Sollima}, A. and {Ferraro}, F.~R. and {Bellazzini}, M.},
    title = "{The mass function of {$\omega$} Centauri down to 0.15 M$_{solar}$}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0708.0721},
 keywords = {methods: observational, techniques: photometric, stars: luminosity function, mass function, globular clusters: individual: {$\omega$} Cen},
     year = 2007,
    month = nov,
   volume = 381,
    pages = {1575-1582},
      doi = {10.1111/j.1365-2966.2007.12324.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.381.1575S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{li2016,
   author = {{Li}, T.~S. and {DePoy}, D.~L. and {Marshall}, J.~L. and {Tucker}, D. and 
	{Kessler}, R. and {Annis}, J. and {Bernstein}, G.~M. and {Boada}, S. and 
	{Burke}, D.~L. and {Finley}, D.~A. and {James}, D.~J. and {Kent}, S. and 
	{Lin}, H. and {Marriner}, J. and {Mondrik}, N. and {Nagasawa}, D. and 
	{Rykoff}, E.~S. and {Scolnic}, D. and {Walker}, A.~R. and {Wester}, W. and 
	{Abbott}, T.~M.~C. and {Allam}, S. and {Benoit-L{\'e}vy}, A. and 
	{Bertin}, E. and {Brooks}, D. and {Capozzi}, D. and {Carnero Rosell}, A. and 
	{Carrasco Kind}, M. and {Carretero}, J. and {Crocce}, M. and 
	{Cunha}, C.~E. and {D'Andrea}, C.~B. and {da Costa}, L.~N. and 
	{Desai}, S. and {Diehl}, H.~T. and {Doel}, P. and {Flaugher}, B. and 
	{Fosalba}, P. and {Frieman}, J. and {Gaztanaga}, E. and {Goldstein}, D.~A. and 
	{Gruen}, D. and {Gruendl}, R.~A. and {Gutierrez}, G. and {Honscheid}, K. and 
	{Kuehn}, K. and {Kuropatkin}, N. and {Maia}, M.~A.~G. and {Melchior}, P. and 
	{Miller}, C.~J. and {Miquel}, R. and {Mohr}, J.~J. and {Neilsen}, E. and 
	{Nichol}, R.~C. and {Nord}, B. and {Ogando}, R. and {Plazas}, A.~A. and 
	{Romer}, A.~K. and {Roodman}, A. and {Sako}, M. and {Sanchez}, E. and 
	{Scarpine}, V. and {Schubnell}, M. and {Sevilla-Noarbe}, I. and 
	{Smith}, R.~C. and {Soares-Santos}, M. and {Sobreira}, F. and 
	{Suchyta}, E. and {Tarle}, G. and {Thomas}, D. and {Vikram}, V. and 
	{DES Collaboration}},
    title = "{Assessment of Systematic Chromatic Errors that Impact Sub-1\% Photometric Precision in Large-area Sky Surveys}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1601.00117},
 primaryClass = "astro-ph.IM",
 keywords = {atmospheric effects, methods: observational, surveys, techniques: photometric},
     year = 2016,
    month = jun,
   volume = 151,
      eid = {157},
    pages = {157},
      doi = {10.3847/0004-6256/151/6/157},
   adsurl = {http://adsabs.harvard.edu/abs/2016AJ....151..157L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{bellini2009,
   author = {{Bellini}, A. and {Piotto}, G. and {Bedin}, L.~R. and {King}, I.~R. and 
	{Anderson}, J. and {Milone}, A.~P. and {Momany}, Y.},
    title = "{Radial distribution of the multiple stellar populations in {$\omega$} Centauri}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0909.4785},
 primaryClass = "astro-ph.SR",
 keywords = {globular clusters: general, globular clusters: individual: {$\omega$} Cen [<ASTROBJ>NGC 5139</ASTROBJ>], stars: evolution, stars: population II, techniques: photometric},
     year = 2009,
    month = dec,
   volume = 507,
    pages = {1393-1408},
      doi = {10.1051/0004-6361/200912757},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...507.1393B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{king2012,
   author = {{King}, I.~R. and {Bedin}, L.~R. and {Cassisi}, S. and {Milone}, A.~P. and 
	{Bellini}, A. and {Piotto}, G. and {Anderson}, J. and {Pietrinferni}, A. and 
	{Cordier}, D.},
    title = "{Hubble Space Telescope Observations of an Outer Field in Omega Centauri: A Definitive Helium Abundance}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1205.3760},
 keywords = {globular clusters: individual: NGC 5139, Hertzsprung-Russell and C-M diagram, proper motions, stars: abundances, stars: Population II},
     year = 2012,
    month = jul,
   volume = 144,
      eid = {5},
    pages = {5},
      doi = {10.1088/0004-6256/144/1/5},
   adsurl = {http://adsabs.harvard.edu/abs/2012AJ....144....5K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{rey2004,
   author = {{Rey}, S.-C. and {Lee}, Y.-W. and {Ree}, C.~H. and {Joo}, J.-M. and 
	{Sohn}, Y.-J. and {Walker}, A.~R.},
    title = "{CCD Photometry of the Globular Cluster {$\omega$} Centauri. II. Stellar Populations and Age-Metallicity Relation}",
  journal = {\aj},
   eprint = {astro-ph/0310773},
 keywords = {Stars: Color-Magnitude Diagrams, Galaxy: Globular Clusters: General, Galaxy: Globular Clusters: Individual: Name: {$\omega$} Centauri},
     year = 2004,
    month = feb,
   volume = 127,
    pages = {958-979},
      doi = {10.1086/380942},
   adsurl = {http://adsabs.harvard.edu/abs/2004AJ....127..958R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{jurcsik1998,
   author = {{Jurcsik}, J.},
    title = "{Spatial Metallicity Asymmetry in {$\omega$} Centauri}",
  journal = {\apjl},
   eprint = {astro-ph/9808327},
 keywords = {GALAXY: GLOBULAR CLUSTERS: INDIVIDUAL: NAME: OMEGA CENTAURI, STARS: ABUNDANCES, STARS: FUNDAMENTAL PARAMETERS, STARS: POPULATION II, STARS: VARIABLES: OTHER, Galaxy: Globular Clusters: Individual: Name: {$\omega$} Centauri, Stars: Abundances, Stars: Fundamental Parameters, Stars: Population II, Stars: Variables: Other},
     year = 1998,
    month = oct,
   volume = 506,
    pages = {L113-L116},
      doi = {10.1086/311648},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...506L.113J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hilker2004,
   author = {{Hilker}, M. and {Kayser}, A. and {Richtler}, T. and {Willemsen}, P.
	},
    title = "{The extended star formation history of {$\omega$} Centauri}",
  journal = {\aap},
   eprint = {astro-ph/0406017},
 keywords = {stars: abundances, globular clusters: individual: {$\omega$} Cen, M 55, galaxies: dwarf, galaxies: nuclei},
     year = 2004,
    month = jul,
   volume = 422,
    pages = {L9-L12},
      doi = {10.1051/0004-6361:20040188},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...422L...9H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{busso2001,
   author = {{Busso}, M. and {Gallino}, R. and {Lambert}, D.~L. and {Travaglio}, C. and 
	{Smith}, V.~V.},
    title = "{Nucleosynthesis and Mixing on the Asymptotic Giant Branch. III. Predicted and Observed s-Process Abundances}",
  journal = {\apj},
   eprint = {astro-ph/0104424},
 keywords = {Nuclear Reactions, Nucleosynthesis, Abundances, Stars: AGB and Post-AGB, Stars: Evolution, Stars: Low-Mass, Brown Dwarfs},
     year = 2001,
    month = aug,
   volume = 557,
    pages = {802-821},
      doi = {10.1086/322258},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...557..802B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{castellani1990,
   author = {{Castellani}, V. and {Chieffi}, A. and {Straniero}, O.},
    title = "{The evolution of intermediate-mass stars through the H- and He-burning phases}",
  journal = {\apjs},
 keywords = {Globular Clusters, Helium, Hydrogen, Nuclear Astrophysics, Stellar Evolution, Stellar Mass, Computational Astrophysics, Hertzsprung-Russell Diagram, Stellar Luminosity, Stellar Models},
     year = 1990,
    month = oct,
   volume = 74,
    pages = {463-499},
      doi = {10.1086/191506},
   adsurl = {http://adsabs.harvard.edu/abs/1990ApJS...74..463C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanture2002,
   author = {{Vanture}, A.~D. and {Wallerstein}, G. and {Suntzeff}, N.~B.
	},
    title = "{Abundance Patterns of the S Stars in {$\omega$} Centauri}",
  journal = {\apj},
 keywords = {Galaxy: Globular Clusters: Individual: Name: {$\omega$} Centauri, Stars: Abundances, Stars: Chemically Peculiar, Stars: Evolution},
     year = 2002,
    month = apr,
   volume = 569,
    pages = {984-996},
      doi = {10.1086/339427},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...569..984V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cunha2002,
   author = {{Cunha}, K. and {Smith}, V.~V. and {Suntzeff}, N.~B. and {Norris}, J.~E. and 
	{Da Costa}, G.~S. and {Plez}, B.},
    title = "{The Evolution of Copper in the Globular Cluster {$\omega$} Centauri}",
  journal = {\aj},
   eprint = {astro-ph/0203408},
 keywords = {Galaxy: Globular Clusters: Individual: Name: {$\omega$} Centauri, Galaxy: Globular Clusters: Individual: NGC Number: NGC 288, Galaxy: Globular Clusters: Individual: NGC Number: NGC 362, Galaxy: Globular Clusters: Individual: NGC Number: NGC 3201, globular clusters: individual (NGC 6752, M4)},
     year = 2002,
    month = jul,
   volume = 124,
    pages = {379-388},
      doi = {10.1086/340967},
   adsurl = {http://adsabs.harvard.edu/abs/2002AJ....124..379C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lee1999,
   author = {{Lee}, Y.-W. and {Joo}, J.-M. and {Sohn}, Y.-J. and {Rey}, S.-C. and 
	{Lee}, H.-C. and {Walker}, A.~R.},
    title = "{Multiple stellar populations in the globular cluster {$\omega$} Centauri as tracers of a merger event}",
  journal = {\nat},
   eprint = {astro-ph/9911137},
     year = 1999,
    month = nov,
   volume = 402,
    pages = {55-57},
      doi = {10.1038/46985},
   adsurl = {http://adsabs.harvard.edu/abs/1999Natur.402...55L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{rey2000,
   author = {{Rey}, S.-C. and {Lee}, Y.-W. and {Joo}, J.-M. and {Walker}, A. and 
	{Baird}, S.},
    title = "{CCD Photometry of the Globular Cluster {$\omega$} Centauri. I. Metallicity of RR Lyrae Stars from CABY Photometry}",
  journal = {\aj},
   eprint = {astro-ph/0001101},
 keywords = {GALAXY: GLOBULAR CLUSTERS: INDIVIDUAL: NAME: {$\Omega$} CENTAURI, STARS: VARIABLES: RR LYRAE VARIABLE, STARS: ABUNDANCES, STARS: HORIZONTAL-BRANCH},
     year = 2000,
    month = apr,
   volume = 119,
    pages = {1824-1838},
      doi = {10.1086/301304},
   adsurl = {http://adsabs.harvard.edu/abs/2000AJ....119.1824R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cannon1973,
   author = {{Cannon}, R.~D. and {Stobie}, R.~S.},
    title = "{Photometry of southern globular clusters I. Bright stars in omega Centauri}",
  journal = {\mnras},
     year = 1973,
   volume = 162,
    pages = {207},
      doi = {10.1093/mnras/162.3.207},
   adsurl = {http://adsabs.harvard.edu/abs/1973MNRAS.162..207C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dickens1967,
   author = {{Dickens}, R.~J. and {Woolley}, R.~v.~d.~R.},
    title = "{Studies of the globular cluster [omega] Centauri V,}",
  journal = {Royal Greenwich Observatory Bulletins},
 keywords = {STARS: GLOBULAR CLUSTERS, HR DIAGRAMS},
     year = 1967,
   volume = 128,
    pages = {255-331},
   adsurl = {http://adsabs.harvard.edu/abs/1967RGOB..128..255D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{villanova2007,
   author = {{Villanova}, S. and {Piotto}, G. and {King}, I.~R. and {Anderson}, J. and 
	{Bedin}, L.~R. and {Gratton}, R.~G. and {Cassisi}, S. and {Momany}, Y. and 
	{Bellini}, A. and {Cool}, A.~M. and {Recio-Blanco}, A. and {Renzini}, A.
	},
    title = "{The Multiplicity of the Subgiant Branch of {$\omega$} Centauri: Evidence for Prolonged Star Formation}",
  journal = {\apj},
   eprint = {astro-ph/0703208},
 keywords = {Galaxy: Abundances, Galaxy: Globular Clusters: Individual: NGC Number: NGC 5139, Stars: Hertzsprung-Russell Diagram},
     year = 2007,
    month = jul,
   volume = 663,
    pages = {296-314},
      doi = {10.1086/517905},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...663..296V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kayser2006,
   author = {{Kayser}, A. and {Hilker}, M. and {Richtler}, T. and {Willemsen}, P.~G.
	},
    title = "{Medium resolution spectroscopy in {$\omega$} Centauri: abundances of 400 subgiant and turn-off region stars}",
  journal = {\aap},
   eprint = {astro-ph/0611286},
 keywords = {stars: abundances, Galaxy: globular clusters: individual: {$\omega$} Cen, galaxies: dwarf, galaxies: nuclei},
     year = 2006,
    month = nov,
   volume = 458,
    pages = {777-788},
      doi = {10.1051/0004-6361:20054462},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...458..777K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{suntzeff1996,
   author = {{Suntzeff}, N.~B. and {Kraft}, R.~P.},
    title = "{The Abundance Spread Among Giants and Subgiants in the Globular Cluster Omega Centauri}",
  journal = {\aj},
   eprint = {astro-ph/9601013},
 keywords = {GLOBULAR CLUSTERS: INDIVIDUAL: OMEGA CENTAURI, STARS: ABUNDANCES, STARS: GIANTS},
     year = 1996,
    month = may,
   volume = 111,
    pages = {1913},
      doi = {10.1086/117930},
   adsurl = {http://adsabs.harvard.edu/abs/1996AJ....111.1913S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{norris1996,
   author = {{Norris}, J.~E. and {Freeman}, K.~C. and {Mighell}, K.~J.},
    title = "{The Giant Branch of omega Centauri. V. The Calcium Abundance Distribution}",
  journal = {\apj},
 keywords = {GALAXY: GLOBULAR CLUSTERS: INDIVIDUAL NAME: OMEGA CENTAURI, STARS: ABUNDANCES, STARS: LATE-TYPE, STARS: POPULATION II},
     year = 1996,
    month = may,
   volume = 462,
    pages = {241},
      doi = {10.1086/177145},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...462..241N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{norris_dacosta1995,
   author = {{Norris}, J.~E. and {Da Costa}, G.~S.},
    title = "{The Giant Branch of omega Centauri. IV. Abundance Patterns Based on Echelle Spectra of 40 Red Giants}",
  journal = {\apj},
 keywords = {GALAXY: GLOBULAR CLUSTERS: INDIVIDUAL NAME: OMEGA CENTAURI, NUCLEAR REACTIONS, NUCLEOSYNTHESIS, ABUNDANCES, STARS: ABUNDANCES, STARS: LATE-TYPE, STARS: POPULATION II},
     year = 1995,
    month = jul,
   volume = 447,
    pages = {680},
      doi = {10.1086/175909},
   adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...447..680N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sollima2005a,
   author = {{Sollima}, A. and {Ferraro}, F.~R. and {Pancino}, E. and {Bellazzini}, M.
	},
    title = "{On the discrete nature of the red giant branch of {$\omega$} Centauri}",
  journal = {\mnras},
   eprint = {astro-ph/0411546},
 keywords = {techniques: photometric, stars: evolution, stars: Population II, globular clusters: individual: {$\omega$} Centauri},
     year = 2005,
    month = feb,
   volume = 357,
    pages = {265-274},
      doi = {10.1111/j.1365-2966.2005.08646.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.357..265S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{vanleeuwen2000,
   author = {{van Leeuwen}, F. and {Le Poole}, R.~S. and {Reijns}, R.~A. and 
	{Freeman}, K.~C. and {de Zeeuw}, P.~T.},
    title = "{A proper motion study of the globular cluster {$\omega$} Centauri}",
  journal = {\aap},
 keywords = {TELESCOPES, CELESTIAL MECHANICS, STELLAR DYNAMICS, GALAXY: GLOBULAR CLUSTERS: INDIVIDUAL: NGC 5139},
     year = 2000,
    month = aug,
   volume = 360,
    pages = {472-498},
   adsurl = {http://adsabs.harvard.edu/abs/2000A%26A...360..472V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{vandeven2006,
   author = {{van de Ven}, G. and {van den Bosch}, R.~C.~E. and {Verolme}, E.~K. and 
	{de Zeeuw}, P.~T.},
    title = "{The dynamical distance and intrinsic structure of the globular cluster {$\omega$} Centauri}",
  journal = {\aap},
   eprint = {astro-ph/0509228},
 keywords = {Galaxy: globular clusters: individual: NGC 5139, Galaxy:, kinematics and dynamics},
     year = 2006,
    month = jan,
   volume = 445,
    pages = {513-543},
      doi = {10.1051/0004-6361:20053061},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...445..513V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{cutri2003,
   author = {{Cutri}, R.~M. and {Skrutskie}, M.~F. and {van Dyk}, S. and 
	{Beichman}, C.~A. and {Carpenter}, J.~M. and {Chester}, T. and 
	{Cambresy}, L. and {Evans}, T. and {Fowler}, J. and {Gizis}, J. and 
	{Howard}, E. and {Huchra}, J. and {Jarrett}, T. and {Kopan}, E.~L. and 
	{Kirkpatrick}, J.~D. and {Light}, R.~M. and {Marsh}, K.~A. and 
	{McCallon}, H. and {Schneider}, S. and {Stiening}, R. and {Sykes}, M. and 
	{Weinberg}, M. and {Wheaton}, W.~A. and {Wheelock}, S. and {Zacarias}, N.
	},
    title = "{VizieR Online Data Catalog: 2MASS All-Sky Catalog of Point Sources (Cutri+ 2003)}",
  journal = {VizieR Online Data Catalog},
 keywords = {Infrared sources, Photometry: infrared, Surveys},
     year = 2003,
    month = jun,
   volume = 2246,
   adsurl = {http://adsabs.harvard.edu/abs/2003yCat.2246....0C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hilker2000,
   author = {{Hilker}, M. and {Richtler}, T.},
    title = "{{$\omega$} Centauri - a former nucleus of a dissolved dwarf galaxy? New evidence from Str{\"o}mgren photometry}",
  journal = {\aap},
   eprint = {astro-ph/0008500},
 keywords = {STARS: ABUNDANCES, GALAXY: GLOBULAR CLUSTERS: GENERAL, GALAXY: GLOBULAR CLUSTERS: INDIVIDUAL: OMEGA CEN, GALAXIES: DWARF, GALAXIES: STELLAR CONTENT},
     year = 2000,
    month = oct,
   volume = 362,
    pages = {895-909},
   adsurl = {http://adsabs.harvard.edu/abs/2000A%26A...362..895H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pancino2007,
   author = {{Pancino}, E. and {Galfo}, A. and {Ferraro}, F.~R. and {Bellazzini}, M.
	},
    title = "{The Rotation of Subpopulations in {$\omega$} Centauri}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0704.2962},
 keywords = {Galaxy: Globular Clusters: Individual: NGC Number: NGC 5139, Techniques: Radial Velocities},
     year = 2007,
    month = jun,
   volume = 661,
    pages = {L155-L158},
      doi = {10.1086/518959},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...661L.155P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{pancino2003,
   author = {{Pancino}, E. and {Seleznev}, A. and {Ferraro}, F.~R. and {Bellazzini}, M. and 
	{Piotto}, G.},
    title = "{The multiple stellar population in {$\omega$} Centauri: spatial distribution and structural properties}",
  journal = {\mnras},
   eprint = {astro-ph/0305524},
 keywords = {globular clusters: individual: NGC 5139},
     year = 2003,
    month = oct,
   volume = 345,
    pages = {683-690},
      doi = {10.1046/j.1365-8711.2003.06981.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.345..683P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{pancino2000,
   author = {{Pancino}, E. and {Ferraro}, F.~R. and {Bellazzini}, M. and 
	{Piotto}, G. and {Zoccali}, M.},
    title = "{New Evidence for the Complex Structure of the Red Giant Branch in {$\omega$} Centauri}",
  journal = {\apjl},
   eprint = {astro-ph/0003222},
 keywords = {GALAXY: GLOBULAR CLUSTERS: INDIVIDUAL: NAME: {$\omega$} CENTAURI, STARS: EVOLUTION},
     year = 2000,
    month = may,
   volume = 534,
    pages = {L83-L87},
      doi = {10.1086/312658},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...534L..83P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{bellini2010,
   author = {{Bellini}, A. and {Bedin}, L.~R. and {Piotto}, G. and {Milone}, A.~P. and 
	{Marino}, A.~F. and {Villanova}, S.},
    title = "{New Hubble Space Telescope WFC3/UVIS Observations Augment the Stellar-population Complexity of {$\omega$} Centauri}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1006.4157},
 keywords = {catalogs, globular clusters: individual: NGC 5139, Hertzsprung-Russell and C-M diagrams, stars: Population II},
     year = 2010,
    month = aug,
   volume = 140,
    pages = {631-641},
      doi = {10.1088/0004-6256/140/2/631},
   adsurl = {http://adsabs.harvard.edu/abs/2010AJ....140..631B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sollima2007a,
   author = {{Sollima}, A. and {Ferraro}, F.~R. and {Bellazzini}, M. and 
	{Origlia}, L. and {Straniero}, O. and {Pancino}, E.},
    title = "{Deep FORS1 Observations of the Double Main Sequence of {$\omega$} Centauri}",
  journal = {\apj},
   eprint = {astro-ph/0609650},
 keywords = {Galaxy: Globular Clusters: Individual: Name: {$\omega$} Centauri, Stars: Evolution, Stars: Population II, Techniques: Photometric},
     year = 2007,
    month = jan,
   volume = 654,
    pages = {915-922},
      doi = {10.1086/509711},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...654..915S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{anderson2002,
   author = {{Anderson}, J.},
    title = "{Main-Sequence Observations with HST}",
booktitle = {Omega Centauri, A Unique Window into Astrophysics},
     year = 2002,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 265,
   editor = {{van Leeuwen}, F. and {Hughes}, J.~D. and {Piotto}, G.},
    pages = {87},
   adsurl = {http://adsabs.harvard.edu/abs/2002ASPC..265...87A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{bedin2004,
   author = {{Bedin}, L.~R. and {Piotto}, G. and {Anderson}, J. and {Cassisi}, S. and 
	{King}, I.~R. and {Momany}, Y. and {Carraro}, G.},
    title = "{{$\omega$} Centauri: The Population Puzzle Goes Deeper}",
  journal = {\apjl},
   eprint = {astro-ph/0403112},
 keywords = {Galaxy: Globular Clusters: Individual: Name: {$\omega$} Centauri, Stars: Hertzsprung-Russell Diagram},
     year = 2004,
    month = apr,
   volume = 605,
    pages = {L125-L128},
      doi = {10.1086/420847},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...605L.125B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{piotto2005,
   author = {{Piotto}, G. and {Villanova}, S. and {Bedin}, L.~R. and {Gratton}, R. and 
	{Cassisi}, S. and {Momany}, Y. and {Recio-Blanco}, A. and {Lucatello}, S. and 
	{Anderson}, J. and {King}, I.~R. and {Pietrinferni}, A. and 
	{Carraro}, G.},
    title = "{Metallicities on the Double Main Sequence of {$\omega$} Centauri Imply Large Helium Enhancement}",
  journal = {\apj},
   eprint = {astro-ph/0412016},
 keywords = {Galaxy: Abundances, Galaxy: Globular Clusters: Individual: NGC Number: NGC 5139, Stars: Hertzsprung-Russell Diagram},
     year = 2005,
    month = mar,
   volume = 621,
    pages = {777-784},
      doi = {10.1086/427796},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...621..777P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{braga2016,
   author = {{Braga}, V.~F. and {Stetson}, P.~B. and {Bono}, G. and {Dall'Ora}, M. and 
	{Ferraro}, I. and {Fiorentino}, G. and {Freyhammer}, L.~M. and 
	{Iannicola}, G. and {Marengo}, M. and {Neeley}, J. and {Valenti}, E. and 
	{Buonanno}, R. and {Calamida}, A. and {Castellani}, M. and {da Silva}, R. and 
	{Degl'Innocenti}, S. and {Di Cecco}, A. and {Fabrizio}, M. and 
	{Freedman}, W.~L. and {Giuffrida}, G. and {Lub}, J. and {Madore}, B.~F. and 
	{Marconi}, M. and {Marinoni}, S. and {Matsunaga}, N. and {Monelli}, M. and 
	{Persson}, S.~E. and {Piersimoni}, A.~M. and {Pietrinferni}, A. and 
	{Prada-Moroni}, P. and {Pulone}, L. and {Stellingwerf}, R. and 
	{Tognelli}, E. and {Walker}, A.~R.},
    title = "{On the RR Lyrae Stars in Globulars. IV. {$\omega$} Centauri Optical UBVRI Photometry}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1609.04916},
 primaryClass = "astro-ph.SR",
 keywords = {globular clusters: individual: omega Cen, stars: distances, stars: horizontal-branch, stars: variables: RR Lyrae},
     year = 2016,
    month = dec,
   volume = 152,
      eid = {170},
    pages = {170},
      doi = {10.3847/0004-6256/152/6/170},
   adsurl = {http://adsabs.harvard.edu/abs/2016AJ....152..170B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{dicecco2015,
   author = {{Di Cecco}, A. and {Bono}, G. and {Prada Moroni}, P.~G. and 
	{Tognelli}, E. and {Allard}, F. and {Stetson}, P.~B. and {Buonanno}, R. and 
	{Ferraro}, I. and {Iannicola}, G. and {Monelli}, M. and {Nonino}, M. and 
	{Pulone}, L.},
    title = "{On the Absolute Age of the Metal-rich Globular M71 (NGC 6838). I. Optical Photometry}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1506.01180},
 primaryClass = "astro-ph.SR",
 keywords = {globular clusters: individual: M71},
     year = 2015,
    month = aug,
   volume = 150,
      eid = {51},
    pages = {51},
      doi = {10.1088/0004-6256/150/2/51},
   adsurl = {http://adsabs.harvard.edu/abs/2015AJ....150...51D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{johnson2010,
   author = {{Johnson}, C.~I. and {Pilachowski}, C.~A.},
    title = "{Chemical Abundances for 855 Giants in the Globular Cluster Omega Centauri (NGC 5139)}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1008.2232},
 primaryClass = "astro-ph.SR",
 keywords = {globular clusters: general, globular clusters: individual: Omega Centauri, stars: abundances, stars: Population II},
     year = 2010,
    month = oct,
   volume = 722,
    pages = {1373-1410},
      doi = {10.1088/0004-637X/722/2/1373},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...722.1373J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{calamida2005,
   author = {{Calamida}, A. and {Stetson}, P.~B. and {Bono}, G. and {Freyhammer}, L.~M. and 
	{Grundahl}, F. and {Hilker}, M. and {Andersen}, M.~I. and {Buonanno}, R. and 
	{Cassisi}, S. and {Corsi}, C.~E. and {Dall'Ora}, M. and {Del Principe}, M. and 
	{Ferraro}, I. and {Monelli}, M. and {Munteanu}, A. and {Nonino}, M. and 
	{Piersimoni}, A.~M. and {Pietrinferni}, A. and {Pulone}, L. and 
	{Richtler}, T.},
    title = "{Reddening Distribution across the Center of the Globular Cluster {$\omega$} Centauri}",
  journal = {\apjl},
   eprint = {astro-ph/0510343},
 keywords = {Galaxy: Globular Clusters: General, Galaxy: Globular Clusters: Individual: Name: {$\omega$} Centauri},
     year = 2005,
    month = nov,
   volume = 634,
    pages = {L69-L72},
      doi = {10.1086/498691},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...634L..69C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{bono2008,
   author = {{Bono}, G. and {Stetson}, P.~B. and {Sanna}, N. and {Piersimoni}, A. and 
	{Freyhammer}, L.~M. and {Bouzid}, Y. and {Buonanno}, R. and 
	{Calamida}, A. and {Caputo}, F. and {Corsi}, C.~E. and {Di Cecco}, A. and 
	{Dall'Ora}, M. and {Ferraro}, I. and {Iannicola}, G. and {Monelli}, M. and 
	{Nonino}, M. and {Pulone}, L. and {Sterken}, C. and {Storm}, J. and 
	{Tuvikene}, T. and {Walker}, A.~R.},
    title = "{On the Relative Distances of {$\omega$} Centauri and 47 Tucanae}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0809.0863},
 keywords = {globular clusters: general, globular clusters: individual: {$\omega$} Centauri 47 Tucanae},
     year = 2008,
    month = oct,
   volume = 686,
      eid = {L87},
    pages = {L87},
      doi = {10.1086/593013},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...686L..87B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{calamida2009,
   author = {{Calamida}, A. and {Bono}, G. and {Stetson}, P.~B. and {Freyhammer}, L.~M. and 
	{Piersimoni}, A.~M. and {Buonanno}, R. and {Caputo}, F. and 
	{Cassisi}, S. and {Castellani}, M. and {Corsi}, C.~E. and {Dall'Ora}, M. and 
	{Degl'Innocenti}, S. and {Ferraro}, I. and {Grundahl}, F. and 
	{Hilker}, M. and {Iannicola}, G. and {Monelli}, M. and {Nonino}, M. and 
	{Patat}, N. and {Pietrinferni}, A. and {Prada Moroni}, P.~G. and 
	{Primas}, F. and {Pulone}, L. and {Richtler}, T. and {Romaniello}, M. and 
	{Storm}, J. and {Walker}, A.~R.},
    title = "{Str{\"o}mgren Photometry of Galactic Globular Clusters. II. Metallicity Distribution of Red Giants in {$\omega$} Centauri}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0909.4661},
 primaryClass = "astro-ph.SR",
 keywords = {globular clusters: general, globular clusters: individual: Omega Centauri, stars: abundances, stars: evolution},
     year = 2009,
    month = dec,
   volume = 706,
    pages = {1277-1298},
      doi = {10.1088/0004-637X/706/2/1277},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...706.1277C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{fukugita1996,
   author = {{Fukugita}, M. and {Ichikawa}, T. and {Gunn}, J.~E. and {Doi}, M. and 
	{Shimasaku}, K. and {Schneider}, D.~P.},
    title = "{The Sloan Digital Sky Survey Photometric System}",
  journal = {\aj},
 keywords = {SURVEYS, INSTRUMENTATION: PHOTOMETERS, TECHNIQUES: PHOTOMETRIC},
     year = 1996,
    month = apr,
   volume = 111,
    pages = {1748},
      doi = {10.1086/117915},
   adsurl = {http://adsabs.harvard.edu/abs/1996AJ....111.1748F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{marconi2014,
   author = {{Marconi}, M. and {Musella}, I. and {Di Criscienzo}, M. and 
	{Cignoni}, M. and {Dall'Ora}, M. and {Bono}, G. and {Ripepi}, V. and 
	{Brocato}, E. and {Raimondo}, G. and {Grado}, A. and {Limatola}, L. and 
	{Coppola}, G. and {Moretti}, M.~I. and {Stetson}, P.~B. and 
	{Calamida}, A. and {Cantiello}, M. and {Capaccioli}, M. and 
	{Cappellaro}, E. and {Cioni}, M.-R.~L. and {Degl'Innocenti}, S. and 
	{De Martino}, D. and {Di Cecco}, A. and {Ferraro}, I. and {Iannicola}, G. and 
	{Prada Moroni}, P.~G. and {Silvotti}, R. and {Buonanno}, R. and 
	{Getman}, F. and {Napolitano}, N.~R. and {Pulone}, L. and {Schipani}, P.
	},
    title = "{STREGA: STRucture and Evolution of the GAlaxy - I. Survey overview and first results}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1406.4375},
 primaryClass = "astro-ph.SR",
 keywords = {Hertzsprung-Russell and colour-magnitude diagrams, globular clusters: individual: NGC 5139, Galaxy: halo, Galaxy: structure},
     year = 2014,
    month = nov,
   volume = 444,
    pages = {3809-3828},
      doi = {10.1093/mnras/stu1691},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.444.3809M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{tonry2012,
   author = {{Tonry}, J.~L. and {Stubbs}, C.~W. and {Lykke}, K.~R. and {Doherty}, P. and 
	{Shivvers}, I.~S. and {Burgett}, W.~S. and {Chambers}, K.~C. and 
	{Hodapp}, K.~W. and {Kaiser}, N. and {Kudritzki}, R.-P. and 
	{Magnier}, E.~A. and {Morgan}, J.~S. and {Price}, P.~A. and 
	{Wainscoat}, R.~J.},
    title = "{The Pan-STARRS1 Photometric System}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1203.0297},
 primaryClass = "astro-ph.IM",
 keywords = {atmospheric effects, instrumentation: photometers, surveys, techniques: photometric},
     year = 2012,
    month = may,
   volume = 750,
      eid = {99},
    pages = {99},
      doi = {10.1088/0004-637X/750/2/99},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...750...99T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{saha2010,
   author = {{Saha}, A. and {Olszewski}, E.~W. and {Brondel}, B. and {Olsen}, K. and 
	{Knezek}, P. and {Harris}, J. and {Smith}, C. and {Subramaniam}, A. and 
	{Claver}, J. and {Rest}, A. and {Seitzer}, P. and {Cook}, K.~H. and 
	{Minniti}, D. and {Suntzeff}, N.~B.},
    title = "{First Results from the NOAO Survey of the Outer Limits of the Magellanic Clouds}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1008.3727},
 keywords = {galaxies: evolution, galaxies: halos, galaxies: structure, Magellanic Clouds, techniques: photometric},
     year = 2010,
    month = dec,
   volume = 140,
    pages = {1719-1738},
      doi = {10.1088/0004-6256/140/6/1719},
   adsurl = {http://adsabs.harvard.edu/abs/2010AJ....140.1719S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{scolnic2015,
   author = {{Scolnic}, D. and {Casertano}, S. and {Riess}, A. and {Rest}, A. and 
	{Schlafly}, E. and {Foley}, R.~J. and {Finkbeiner}, D. and {Tang}, C. and 
	{Burgett}, W.~S. and {Chambers}, K.~C. and {Draper}, P.~W. and 
	{Flewelling}, H. and {Hodapp}, K.~W. and {Huber}, M.~E. and 
	{Kaiser}, N. and {Kudritzki}, R.~P. and {Magnier}, E.~A. and 
	{Metcalfe}, N. and {Stubbs}, C.~W.},
    title = "{Supercal: Cross-calibration of Multiple Photometric Systems to Improve Cosmological Measurements with Type Ia Supernovae}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1508.05361},
 primaryClass = "astro-ph.IM",
 keywords = {dark energy, supernovae: general, surveys},
     year = 2015,
    month = dec,
   volume = 815,
      eid = {117},
    pages = {117},
      doi = {10.1088/0004-637X/815/2/117},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...815..117S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{castellani2007,
   author = {{Castellani}, V. and {Calamida}, A. and {Bono}, G. and {Stetson}, P.~B. and 
	{Freyhammer}, L.~M. and {Degl'Innocenti}, S. and {Moroni}, P.~P. and 
	{Monelli}, M. and {Corsi}, C.~E. and {Nonino}, M. and {Buonanno}, R. and 
	{Caputo}, F. and {Castellani}, M. and {Dall'Ora}, M. and {Del Principe}, M. and 
	{Ferraro}, I. and {Iannicola}, G. and {Piersimoni}, A.~M. and 
	{Pulone}, L. and {Vuerli}, C.},
    title = "{Star Counts in the Globular Cluster {$\omega$} Centauri. I. Bright Stellar Components}",
  journal = {\apj},
   eprint = {astro-ph/0703401},
 keywords = {Galaxy: Globular Clusters: Individual: Name: {$\omega$} Centauri, Stars: Evolution, Stars: Horizontal-Branch},
     year = 2007,
    month = jul,
   volume = 663,
    pages = {1021-1039},
      doi = {10.1086/518209},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...663.1021C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{rest05,
   author = {{Rest}, A. and {Stubbs}, C. and {Becker}, A.~C. and {Miknaitis}, G.~A. and 
    {Miceli}, A. and {Covarrubias}, R. and {Hawley}, S.~L. and {Smith}, R.~C. and 
    {Suntzeff}, N.~B. and {Olsen}, K. and {Prieto}, J.~L. and {Hiriart}, R. and 
    {Welch}, D.~L. and {Cook}, K.~H. and {Nikolaev}, S. and {Huber}, M. and 
    {Prochtor}, G. and {Clocchiatti}, A. and {Minniti}, D. and {Garg}, A. and 
    {Challis}, P. and {Keller}, S.~C. and {Schmidt}, B.~P.},
    title = "{Testing LMC Microlensing Scenarios: The Discrimination Power of the SuperMACHO Microlensing Survey}",
  journal = {\apj},
   eprint = {astro-ph/0509240},
 keywords = {Cosmology: Dark Matter, Galaxies: Halos, Galaxies: Structure, Galaxy: Structure, Cosmology: Gravitational Lensing, Galaxies: Magellanic Clouds},
     year = 2005,
    month = dec,
   volume = 634,
    pages = {1103-1115},
      doi = {10.1086/497060},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...634.1103R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{rest14,
   author = {{Rest}, A. and {Scolnic}, D. and {Foley}, R.~J. and {Huber}, M.~E. and 
    {Chornock}, R. and {Narayan}, G. and {Tonry}, J.~L. and {Berger}, E. and 
    {Soderberg}, A.~M. and {Stubbs}, C.~W. and {Riess}, A. and {Kirshner}, R.~P. and 
    {Smartt}, S.~J. and {Schlafly}, E. and {Rodney}, S. and {Botticella}, M.~T. and 
    {Brout}, D. and {Challis}, P. and {Czekala}, I. and {Drout}, M. and 
    {Hudson}, M.~J. and {Kotak}, R. and {Leibler}, C. and {Lunnan}, R. and 
    {Marion}, G.~H. and {McCrum}, M. and {Milisavljevic}, D. and 
    {Pastorello}, A. and {Sanders}, N.~E. and {Smith}, K. and {Stafford}, E. and 
    {Thilker}, D. and {Valenti}, S. and {Wood-Vasey}, W.~M. and 
    {Zheng}, Z. and {Burgett}, W.~S. and {Chambers}, K.~C. and {Denneau}, L. and 
    {Draper}, P.~W. and {Flewelling}, H. and {Hodapp}, K.~W. and 
    {Kaiser}, N. and {Kudritzki}, R.-P. and {Magnier}, E.~A. and 
    {Metcalfe}, N. and {Price}, P.~A. and {Sweeney}, W. and {Wainscoat}, R. and 
    {Waters}, C.},
    title = "{Cosmological Constraints from Measurements of Type Ia Supernovae Discovered during the First 1.5 yr of the Pan-STARRS1 Survey}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1310.3828},
 keywords = {cosmological parameters, cosmology: observations, dark energy, supernovae: general},
     year = 2014,
    month = nov,
   volume = 795,
      eid = {44},
    pages = {44},
      doi = {10.1088/0004-637X/795/1/44},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...795...44R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{johnson2013,
   author = {{Johnson}, C.~I. and {Rich}, R.~M. and {Kobayashi}, C. and {Kunder}, A. and 
	{Pilachowski}, C.~A. and {Koch}, A. and {de Propris}, R.},
    title = "{Metallicity Distribution Functions, Radial Velocities, and Alpha Element Abundances in Three Off-axis Bulge Fields}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1302.3679},
 primaryClass = "astro-ph.SR",
 keywords = {Galaxy: bulge, Galaxy: stellar content, stars: abundances, stars: general, stars: Population II},
     year = 2013,
    month = mar,
   volume = 765,
      eid = {157},
    pages = {157},
      doi = {10.1088/0004-637X/765/2/157},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...765..157J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{johnson2011,
   author = {{Johnson}, C.~I. and {Rich}, R.~M. and {Fulbright}, J.~P. and 
	{Valenti}, E. and {McWilliam}, A.},
    title = "{Alpha Enhancement and the Metallicity Distribution Function of Plaut's Window}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1103.2143},
 primaryClass = "astro-ph.SR",
 keywords = {Galaxy: abundances, Galaxy: bulge, stars: abundances, stars: Population II},
     year = 2011,
    month = may,
   volume = 732,
      eid = {108},
    pages = {108},
      doi = {10.1088/0004-637X/732/2/108},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...732..108J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{gonzalez11,
   author = {{Gonzalez}, O.~A. and {Rejkuba}, M. and {Zoccali}, M. and {Hill}, V. and 
	{Battaglia}, G. and {Babusiaux}, C. and {Minniti}, D. and {Barbuy}, B. and 
	{Alves-Brito}, A. and {Renzini}, A. and {Gomez}, A. and {Ortolani}, S.
	},
    title = "{Alpha element abundances and gradients in the Milky Way bulge from FLAMES-GIRAFFE spectra of 650 K giants}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1103.6104},
 keywords = {stars: abundances, stars: late-type, Galaxy: abundances, Galaxy: bulge, Galaxy: formation},
     year = 2011,
    month = jun,
   volume = 530,
      eid = {A54},
    pages = {A54},
      doi = {10.1051/0004-6361/201116548},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...530A..54G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{kroupa97,
   author = {{Kroupa}, P. and {Tout}, C.~A.},
    title = "{The theoretical mass-magnitude relation of low mass stars and its metallicity dependence}",
  journal = {\mnras},
   eprint = {astro-ph/9701213},
     year = 1997,
    month = may,
   volume = 287,
    pages = {402-414},
   adsurl = {http://adsabs.harvard.edu/abs/1997MNRAS.287..402K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bedin09,
   author = {{Bedin}, L.~R. and {Salaris}, M. and {Piotto}, G. and {Anderson}, J. and 
	{King}, I.~R. and {Cassisi}, S.},
    title = "{The End of the White Dwarf Cooling Sequence in M4: An Efficient Approach}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0903.2839},
 primaryClass = "astro-ph.GA",
 keywords = {globular clusters: individual: NGC 6121, white dwarfs},
     year = 2009,
    month = jun,
   volume = 697,
    pages = {965-979},
      doi = {10.1088/0004-637X/697/2/965},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...697..965B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cassisi09,
   author = {{Cassisi}, S. and {Salaris}, M. and {Anderson}, J. and {Piotto}, G. and 
	{Pietrinferni}, A. and {Milone}, A. and {Bellini}, A. and {Bedin}, L.~R.
	},
    title = "{Hot Horizontal Branch Stars in {$\omega$} Centauri: Clues about their Origin from the Cluster Color Magnitude Diagram}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0907.3550},
 primaryClass = "astro-ph.SR",
 keywords = {galaxies: stellar content, globular clusters: general, stars: abundances, stars: evolution, stars: horizontal-branch, white dwarfs},
     year = 2009,
    month = sep,
   volume = 702,
    pages = {1530-1535},
      doi = {10.1088/0004-637X/702/2/1530},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...702.1530C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cassisi11,
   author = {{Cassisi}, S. and {Salaris}, M.},
    title = "{A Classical Cepheid in a Large Magellanic Cloud Eclipsing Binary: Evidence Of Shortcomings in Current Stellar Evolutionary Models?}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1101.0394},
 primaryClass = "astro-ph.SR",
 keywords = {binaries: eclipsing, stars: evolution, stars: fundamental parameters, stars: variables: Cepheids},
     year = 2011,
    month = feb,
   volume = 728,
      eid = {L43},
    pages = {L43},
      doi = {10.1088/2041-8205/728/2/L43},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...728L..43C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cassisi14,
   author = {{Cassisi}, S. and {Salaris}, M. and {Pietrinferni}, A. and {Vink}, J.~S. and 
	{Monelli}, M.},
    title = "{On the missing second generation AGB stars in NGC 6752}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1410.3599},
 primaryClass = "astro-ph.SR",
 keywords = {stars: abundances, stars: AGB and post-AGB, globular clusters: general, galaxies: clusters: individual: NGC 6752, stars: horizontal-branch},
     year = 2014,
    month = nov,
   volume = 571,
      eid = {A81},
    pages = {A81},
      doi = {10.1051/0004-6361/201424540},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...571A..81C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{portail15,
   author = {{Portail}, M. and {Wegg}, C. and {Gerhard}, O. and {Martinez-Valpuesta}, I.
	},
    title = "{Made-to-measure models of the Galactic box/peanut bulge: stellar and total mass in the bulge region}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1502.00633},
 keywords = {methods: numerical, Galaxy: bulge, Galaxy: centre, Galaxy: kinematics and dynamics, Galaxy: structure},
     year = 2015,
    month = mar,
   volume = 448,
    pages = {713-731},
      doi = {10.1093/mnras/stv058},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.448..713P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{bond01,
   author = {{Bond}, I.~A. and {Abe}, F. and {Dodd}, R.~J. and {Hearnshaw}, J.~B. and 
	{Honda}, M. and {Jugaku}, J. and {Kilmartin}, P.~M. and {Marles}, A. and 
	{Masuda}, K. and {Matsubara}, Y. and {Muraki}, Y. and {Nakamura}, T. and 
	{Nankivell}, G. and {Noda}, S. and {Noguchi}, C. and {Ohnishi}, K. and 
	{Rattenbury}, N.~J. and {Reid}, M. and {Saito}, T. and {Sato}, H. and 
	{Sekiguchi}, M. and {Skuljan}, J. and {Sullivan}, D.~J. and 
	{Sumi}, T. and {Takeuti}, M. and {Watase}, Y. and {Wilkinson}, S. and 
	{Yamada}, R. and {Yanagisawa}, T. and {Yock}, P.~C.~M.},
    title = "{Real-time difference imaging analysis of MOA Galactic bulge observations during 2000}",
  journal = {\mnras},
   eprint = {astro-ph/0102181},
 keywords = {GRAVITATIONAL LENSING, TECHNIQUES: IMAGE PROCESSING},
     year = 2001,
    month = nov,
   volume = 327,
    pages = {868-880},
      doi = {10.1046/j.1365-8711.2001.04776.x},
   adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.327..868B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{sako08,
   author = {{Sako}, T. and {Sekiguchi}, T. and {Sasaki}, M. and {Okajima}, K. and 
	{Abe}, F. and {Bond}, I.~A. and {Hearnshaw}, J.~B. and {Itow}, Y. and 
	{Kamiya}, K. and {Kilmartin}, P.~M. and {Masuda}, K. and {Matsubara}, Y. and 
	{Muraki}, Y. and {Rattenbury}, N.~J. and {Sullivan}, D.~J. and 
	{Sumi}, T. and {Tristram}, P. and {Yanagisawa}, T. and {Yock}, P.~C.~M.
	},
    title = "{MOA-cam3: a wide-field mosaic CCD camera for a gravitational microlensing survey in New Zealand}",
  journal = {Experimental Astronomy},
archivePrefix = "arXiv",
   eprint = {0804.0653},
 keywords = {CCD cameras, Wide-field survey telescope, Gravitational microlensing},
     year = 2008,
    month = oct,
   volume = 22,
    pages = {51-66},
      doi = {10.1007/s10686-007-9082-5},
   adsurl = {http://adsabs.harvard.edu/abs/2008ExA....22...51S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{udalski15,
   author = {{Udalski}, A. and {Szyma{\'n}ski}, M.~K. and {Szyma{\'n}ski}, G.
	},
    title = "{OGLE-IV: Fourth Phase of the Optical Gravitational Lensing Experiment}",
  journal = {Acta Astron.},
archivePrefix = "arXiv",
   eprint = {1504.05966},
 primaryClass = "astro-ph.SR",
 keywords = {Surveys, Techniques: Photometric, Galaxy: bulge, Galaxy: disk, Magellanic Clouds},
     year = 2015,
    month = mar,
   volume = 65,
    pages = {1-38},
   adsurl = {http://adsabs.harvard.edu/abs/2015AcA....65....1U},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sofue09,
   author = {{Sofue}, Y. and {Honma}, M. and {Omodaka}, T.},
    title = "{Unified Rotation Curve of the Galaxy -- Decomposition into de Vaucouleurs Bulge, Disk, Dark Halo, and the 9-kpc Rotation Dip --}",
  journal = {\pasj},
archivePrefix = "arXiv",
   eprint = {0811.0859},
 keywords = {Galaxy: bulge, Galaxy: disk, Galaxy: rotation curve, Galaxy: structure},
     year = 2009,
    month = feb,
   volume = 61,
    pages = {227-},
      doi = {10.1093/pasj/61.2.227},
   adsurl = {http://adsabs.harvard.edu/abs/2009PASJ...61..227S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kalirai13,
   author = {{Kalirai}, J.~S. and {Anderson}, J. and {Dotter}, A. and {Richer}, H.~B. and 
	{Fahlman}, G.~G. and {Hansen}, B.~M.~S. and {Hurley}, J. and 
	{Reid}, I.~N. and {Rich}, R.~M. and {Shara}, M.~M.},
    title = "{Ultra-Deep Hubble Space Telescope Imaging of the Small Magellanic Cloud: The Initial Mass Function of Stars with M {\lt}\~{} 1 M $_{⊙}$}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1212.1159},
 primaryClass = "astro-ph.GA",
 keywords = {galaxies: photometry, galaxies: stellar content, Magellanic Clouds, methods: data analysis, methods: statistical, stars: luminosity function, mass function, techniques: photometric},
     year = 2013,
    month = feb,
   volume = 763,
      eid = {110},
    pages = {110},
      doi = {10.1088/0004-637X/763/2/110},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...763..110K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{geha13,
   author = {{Geha}, M. and {Brown}, T.~M. and {Tumlinson}, J. and {Kalirai}, J.~S. and 
	{Simon}, J.~D. and {Kirby}, E.~N. and {VandenBerg}, D.~A. and 
	{Mu{\~n}oz}, R.~R. and {Avila}, R.~J. and {Guhathakurta}, P. and 
	{Ferguson}, H.~C.},
    title = "{The Stellar Initial Mass Function of Ultra-faint Dwarf Galaxies: Evidence for IMF Variations with Galactic Environment}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1304.7769},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: dwarf, galaxies: evolution, galaxies: photometry, galaxies: stellar content, Local Group},
     year = 2013,
    month = jul,
   volume = 771,
      eid = {29},
    pages = {29},
      doi = {10.1088/0004-637X/771/1/29},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...771...29G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{percival09,
   author = {{Percival}, S.~M. and {Salaris}, M. and {Cassisi}, S. and {Pietrinferni}, A.
	},
    title = "{A Large Stellar Evolution Database for Population Synthesis Studies. IV. Integrated Properties and Spectra}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0809.0265},
 keywords = {galaxies: evolution, galaxies: stellar content, stars: evolution},
     year = 2009,
    month = jan,
   volume = 690,
    pages = {427-439},
      doi = {10.1088/0004-637X/690/1/427},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...690..427P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sirianni2005,
   author = {{Sirianni}, M. and {Jee}, M.~J. and {Ben{\'{\i}}tez}, N. and 
	{Blakeslee}, J.~P. and {Martel}, A.~R. and {Meurer}, G. and 
	{Clampin}, M. and {De Marchi}, G. and {Ford}, H.~C. and {Gilliland}, R. and 
	{Hartig}, G.~F. and {Illingworth}, G.~D. and {Mack}, J. and 
	{McCann}, W.~J.},
    title = "{The Photometric Performance and Calibration of the Hubble Space Telescope Advanced Camera for Surveys}",
  journal = {\pasp},
   eprint = {astro-ph/0507614},
 keywords = {Instrumentation: Detectors, Instrumentation: Photometers, Techniques: Photometric, Methods: Data Analysis},
     year = 2005,
    month = oct,
   volume = 117,
    pages = {1049-1112},
      doi = {10.1086/444553},
   adsurl = {http://adsabs.harvard.edu/abs/2005PASP..117.1049S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{nataf13,
   author = {{Nataf}, D.~M. and {Gould}, A. and {Fouqu{\'e}}, P. and {Gonzalez}, O.~A. and 
	{Johnson}, J.~A. and {Skowron}, J. and {Udalski}, A. and {Szyma{\'n}ski}, M.~K. and 
	{Kubiak}, M. and {Pietrzy{\'n}ski}, G. and {Soszy{\'n}ski}, I. and 
	{Ulaczyk}, K. and {Wyrzykowski}, {\L}. and {Poleski}, R.},
    title = "{Reddening and Extinction toward the Galactic Bulge from OGLE-III: The Inner Milky Way's R$_{V}$ \~{} 2.5 Extinction Curve}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1208.1263},
 primaryClass = "astro-ph.GA",
 keywords = {dust, extinction, Galaxy: bulge, Galaxy: fundamental parameters, Galaxy: stellar content, Galaxy: structure},
     year = 2013,
    month = jun,
   volume = 769,
      eid = {88},
    pages = {88},
      doi = {10.1088/0004-637X/769/2/88},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...769...88N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{vazdekis15,
   author = {{Vazdekis}, A. and {Coelho}, P. and {Cassisi}, S. and {Ricciardelli}, E. and 
	{Falc{\'o}n-Barroso}, J. and {S{\'a}nchez-Bl{\'a}zquez}, P. and 
	{Barbera}, F.~L. and {Beasley}, M.~A. and {Pietrinferni}, A.
	},
    title = "{Evolutionary stellar population synthesis with MILES - II. Scaled-solar and {$\alpha$}-enhanced models}",
  journal = {\mnras},
 keywords = {stars: fundamental parameters, globular clusters: general, galaxies: abundances, galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: stellar content},
     year = 2015,
    month = may,
   volume = 449,
    pages = {1177-1214},
      doi = {10.1093/mnras/stv151},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.449.1177V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{hangould96,
   author = {{Han}, C. and {Gould}, A.},
    title = "{Statistical Determination of the MACHO Mass Spectrum}",
  journal = {\apj},
   eprint = {astro-ph/9504078},
 keywords = {COSMOLOGY: GRAVITATIONAL LENSING, COSMOLOGY: DARK MATTER},
     year = 1996,
    month = aug,
   volume = 467,
    pages = {540},
      doi = {10.1086/177631},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...467..540H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{zhao95,
   author = {{Zhao}, H. and {Spergel}, D.~N. and {Rich}, R.~M.},
    title = "{Microlensing by the galactic bar}",
  journal = {\apjl},
   eprint = {astro-ph/9409022},
 keywords = {Astronomical Models, Dark Matter, Galactic Bulge, Gravitational Lenses, Brightness Distribution, Brown Dwarf Stars, Cosmic Background Explorer Satellite, Monte Carlo Method, Probability Distribution Functions},
     year = 1995,
    month = feb,
   volume = 440,
    pages = {L13-L16},
      doi = {10.1086/187749},
   adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...440L..13Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{sumi13,
   author = {{Sumi}, T. and {Bennett}, D.~P. and {Bond}, I.~A. and {Abe}, F. and 
	{Botzler}, C.~S. and {Fukui}, A. and {Furusawa}, K. and {Itow}, Y. and 
	{Ling}, C.~H. and {Masuda}, K. and {Matsubara}, Y. and {Muraki}, Y. and 
	{Ohnishi}, K. and {Rattenbury}, N. and {Saito}, T. and {Sullivan}, D.~J. and 
	{Suzuki}, D. and {Sweatman}, W.~L. and {Tristram}, P.~J. and 
	{Wada}, K. and {Yock}, P.~C.~M. and {MOA Collaboratoin}, T.},
    title = "{The Microlensing Event Rate and Optical Depth toward the Galactic Bulge from MOA-II}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1305.0186},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: bulge, gravitational lensing: micro, stars: luminosity function, mass function},
     year = 2013,
    month = dec,
   volume = 778,
      eid = {150},
    pages = {150},
      doi = {10.1088/0004-637X/778/2/150},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...778..150S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Wyrzykowski15,
   author = {{Wyrzykowski}, {\L}. and {Rynkiewicz}, A.~E. and {Skowron}, J. and 
	{Koz{\l}owski}, S. and {Udalski}, A. and {Szyma{\'n}ski}, M.~K. and 
	{Kubiak}, M. and {Soszy{\'n}ski}, I. and {Pietrzy{\'n}ski}, G. and 
	{Poleski}, R. and {Pietrukowicz}, P. and {Pawlak}, M.},
    title = "{OGLE-III Microlensing Events and the Structure of the Galactic Bulge}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1405.3134},
 primaryClass = "astro-ph.SR",
 keywords = {catalogs, Galaxy: bulge, Galaxy: structure, gravitational lensing: micro},
     year = 2015,
    month = jan,
   volume = 216,
      eid = {12},
    pages = {12},
      doi = {10.1088/0067-0049/216/1/12},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJS..216...12W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Paczynski94,
   author = {{Paczynski}, B. and {Stanek}, K.~Z. and {Udalski}, A. and {Szymanski}, M. and 
	{Kaluzny}, J. and {Kubiak}, M. and {Mateo}, M. and {Krzeminski}, W.
	},
    title = "{Are the OGLE microlenses in the galactic bar?}",
  journal = {\apjl},
   eprint = {astro-ph/9407010},
 keywords = {Astronomical Models, Barred Galaxies, Galactic Bulge, Gravitational Lenses, Mass Distribution, Astronomical Observatories, Brown Dwarf Stars, Charge Coupled Devices, Dark Matter, Galactic Structure, Hubble Space Telescope, Photometry, Spectroscopy, Telescopes},
     year = 1994,
    month = nov,
   volume = 435,
    pages = {L113-L116},
      doi = {10.1086/187607},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...435L.113P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{raghavan10,
   author = {{Raghavan}, D. and {McAlister}, H.~A. and {Henry}, T.~J. and 
	{Latham}, D.~W. and {Marcy}, G.~W. and {Mason}, B.~D. and {Gies}, D.~R. and 
	{White}, R.~J. and {ten Brummelaar}, T.~A.},
    title = "{A Survey of Stellar Families: Multiplicity of Solar-type Stars}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1007.0414},
 primaryClass = "astro-ph.SR",
 keywords = {binaries: general, planetary systems, stars: solar-type, stars: statistics, surveys},
     year = 2010,
    month = sep,
   volume = 190,
    pages = {1-42},
      doi = {10.1088/0067-0049/190/1/1},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJS..190....1R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ozel10,
   author = {{{\"O}zel}, F. and {Psaltis}, D. and {Narayan}, R. and {McClintock}, J.~E.
	},
    title = "{The Black Hole Mass Distribution in the Galaxy}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1006.2834},
 primaryClass = "astro-ph.GA",
 keywords = {black hole physics, X-rays: binaries},
     year = 2010,
    month = dec,
   volume = 725,
    pages = {1918-1927},
      doi = {10.1088/0004-637X/725/2/1918},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...725.1918O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{reid02,
   author = {{Reid}, I.~N. and {Gizis}, J.~E. and {Hawley}, S.~L.},
    title = "{The Palomar/MSU Nearby Star Spectroscopic Survey. IV. The Luminosity Function in the Solar Neighborhood and M Dwarf Kinematics}",
  journal = {\aj},
 keywords = {Galaxy: Solar Neighborhood, Stars: Kinematics, Stars: Luminosity Function, Mass Function},
     year = 2002,
    month = nov,
   volume = 124,
    pages = {2721-2738},
      doi = {10.1086/343777},
   adsurl = {http://adsabs.harvard.edu/abs/2002AJ....124.2721R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{bochanski10,
   author = {{Bochanski}, J.~J. and {Hawley}, S.~L. and {Covey}, K.~R. and 
	{West}, A.~A. and {Reid}, I.~N. and {Golimowski}, D.~A. and 
	{Ivezi{\'c}}, {\v Z}.},
    title = "{The Luminosity and Mass Functions of Low-mass Stars in the Galactic Disk. II. The Field}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1004.4002},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, Galaxy: stellar content, Galaxy: structure, stars: fundamental parameters, stars: late-type, stars: low-mass, stars: luminosity function, mass function},
     year = 2010,
    month = jun,
   volume = 139,
      eid = {2679},
    pages = {2679-2699},
      doi = {10.1088/0004-6256/139/6/2679},
   adsurl = {http://adsabs.harvard.edu/abs/2010AJ....139.2679B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{covey08,
   author = {{Covey}, K.~R. and {Hawley}, S.~L. and {Bochanski}, J.~J. and 
	{West}, A.~A. and {Reid}, I.~N. and {Golimowski}, D.~A. and 
	{Davenport}, J.~R.~A. and {Henry}, T. and {Uomoto}, A. and {Holtzman}, J.~A.
	},
    title = "{The Luminosity and Mass Functions of Low-Mass Stars in the Galactic Disk. I. The Calibration Region}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {0807.2452},
 keywords = {Galaxy: stellar content, stars: late-type, stars: low-mass, brown dwarfs, stars: luminosity function, mass function, surveys},
     year = 2008,
    month = nov,
   volume = 136,
    pages = {1778-1798},
      doi = {10.1088/0004-6256/136/5/1778},
   adsurl = {http://adsabs.harvard.edu/abs/2008AJ....136.1778C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{chabrier05,
   author = {{Chabrier}, G.},
    title = "{The Initial Mass Function: from Salpeter 1955 to 2005}",
booktitle = {The Initial Mass Function 50 Years Later},
     year = 2005,
   series = {Astrophysics and Space Science Library},
   volume = 327,
   eprint = {astro-ph/0409465},
   editor = {{Corbelli}, E. and {Palla}, F. and {Zinnecker}, H.},
    month = jan,
    pages = {41},
   adsurl = {http://adsabs.harvard.edu/abs/2005ASSL..327...41C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dutton13,
   author = {{Dutton}, A.~A. and {Treu}, T. and {Brewer}, B.~J. and {Marshall}, P.~J. and 
	{Auger}, M.~W. and {Barnab{\`e}}, M. and {Koo}, D.~C. and {Bolton}, A.~S. and 
	{Koopmans}, L.~V.~E.},
    title = "{The SWELLS survey - V. A Salpeter stellar initial mass function in the bulges of massive spiral galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1206.4310},
 primaryClass = "astro-ph.CO",
 keywords = {stars: luminosity function, mass function, galaxies: bulges, galaxies: kinematics and dynamics, galaxies: spiral, dark matter},
     year = 2013,
    month = feb,
   volume = 428,
    pages = {3183-3195},
      doi = {10.1093/mnras/sts262},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.428.3183D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kroupa90,
   author = {{Kroupa}, P. and {Tout}, C.~A. and {Gilmore}, G.},
    title = "{The low-luminosity stellar mass function}",
  journal = {\mnras},
 keywords = {Mass To Light Ratios, Stellar Luminosity, Stellar Mass, Astronomical Models, Hydrogen, Stellar Atmospheres, Stellar Magnitude},
     year = 1990,
    month = may,
   volume = 244,
    pages = {76-85},
   adsurl = {http://adsabs.harvard.edu/abs/1990MNRAS.244...76K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{duquennoy91,
   author = {{Duquennoy}, A. and {Mayor}, M.},
    title = "{Multiplicity among solar-type stars in the solar neighbourhood. II - Distribution of the orbital elements in an unbiased sample}",
  journal = {\aap},
 keywords = {Binary Stars, Dwarf Stars, G Stars, Solar Neighborhood, Stellar Orbits, Brown Dwarf Stars, Orbital Elements, Peculiar Stars, Radial Velocity, Stellar Evolution, Variable Stars},
     year = 1991,
    month = aug,
   volume = 248,
    pages = {485-524},
   adsurl = {http://adsabs.harvard.edu/abs/1991A%26A...248..485D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


ARTICLE{paresce00,
   author = {{Paresce}, F. and {De Marchi}, G.},
    title = "{On the Globular Cluster Initial Mass Function below 1 M$_{solar}$}",
  journal = {\apj},
 keywords = {Galaxy: Globular Clusters: General, Stars: Luminosity Function, Mass Function},
     year = 2000,
    month = may,
   volume = 534,
    pages = {870-879},
      doi = {10.1086/308775},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...534..870P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{luhman00,
   author = {{Luhman}, K.~L. and {Rieke}, G.~H. and {Young}, E.~T. and {Cotera}, A.~S. and 
	{Chen}, H. and {Rieke}, M.~J. and {Schneider}, G. and {Thompson}, R.~I.
	},
    title = "{The Initial Mass Function of Low-Mass Stars and Brown Dwarfs in Young Clusters}",
  journal = {\apj},
   eprint = {astro-ph/0004386},
 keywords = {Infrared: Stars, Stars: Evolution, Stars: Formation, Stars: Low-Mass, Brown Dwarfs, Stars: Luminosity Function, Mass Function, Stars: Pre-Main-Sequence},
     year = 2000,
    month = sep,
   volume = 540,
    pages = {1016-1040},
      doi = {10.1086/309365},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...540.1016L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{gould97,
   author = {{Gould}, A. and {Bahcall}, J.~N. and {Flynn}, C.},
    title = "{M Dwarfs from Hubble Space Telescope Star Counts. III. The Groth Strip}",
  journal = {\apj},
   eprint = {astro-ph/9611157},
 keywords = {Stars: Late-Type, stars: low-mass, brown dwarfs -- stars: luminosity function, mass function, Stars: Statistics, Surveys},
     year = 1997,
    month = jun,
   volume = 482,
    pages = {913-918},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...482..913G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{reid97,
   author = {{Reid}, I.~N. and {Gizis}, J.~E.},
    title = "{Low-Mass Binaries and the Stellar Luminosity Function}",
  journal = {\aj},
 keywords = {STARS: LUMINOSITY FUNCTION, STARS: LOW-MASS, BINARIES: GENERAL},
     year = 1997,
    month = jun,
   volume = 113,
    pages = {2246},
      doi = {10.1086/118436},
   adsurl = {http://adsabs.harvard.edu/abs/1997AJ....113.2246R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{salpeter55,
   author = {{Salpeter}, E.~E.},
    title = "{The Luminosity Function and Stellar Evolution.}",
  journal = {\apj},
     year = 1955,
    month = jan,
   volume = 121,
    pages = {161},
      doi = {10.1086/145971},
   adsurl = {http://adsabs.harvard.edu/abs/1955ApJ...121..161S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kroupa93,
   author = {{Kroupa}, P. and {Tout}, C.~A. and {Gilmore}, G.},
    title = "{The distribution of low-mass stars in the Galactic disc}",
  journal = {\mnras},
 keywords = {Binary Stars, Galactic Nuclei, Milky Way Galaxy, Star Distribution, Stellar Mass, Color-Magnitude Diagram, Main Sequence Stars, Mass To Light Ratios, Metallicity, Solar Neighborhood, Stellar Evolution, Stellar Luminosity},
     year = 1993,
    month = jun,
   volume = 262,
    pages = {545-587},
   adsurl = {http://adsabs.harvard.edu/abs/1993MNRAS.262..545K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kroupa01,
   author = {{Kroupa}, P.},
    title = "{On the variation of the initial mass function}",
  journal = {\mnras},
   eprint = {astro-ph/0009005},
 keywords = {BINARIES: GENERAL, STARS: FORMATION, STARS: KINEMATICS, STARS: LUMINOSITY FUNCTION, MASS FUNCTION, GLOBULAR CLUSTERS: GENERAL, OPEN CLUSTERS AND ASSOCIATIONS: GENERAL},
     year = 2001,
    month = apr,
   volume = 322,
    pages = {231-246},
      doi = {10.1046/j.1365-8711.2001.04022.x},
   adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.322..231K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kroupa91,
   author = {{Kroupa}, P. and {Gilmore}, G. and {Tout}, C.~A.},
    title = "{The effects of unresolved binary stars on the determination of the stellar mass function}",
  journal = {\mnras},
 keywords = {Astronomical Photometry, Binary Stars, Stellar Luminosity, Stellar Mass, Brown Dwarf Stars, Galactic Structure, Hertzsprung-Russell Diagram, Monte Carlo Method, Stellar Magnitude},
     year = 1991,
    month = jul,
   volume = 251,
    pages = {293-302},
   adsurl = {http://adsabs.harvard.edu/abs/1991MNRAS.251..293K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kroupa95,
   author = {{Kroupa}, P.},
    title = "{Are the nearby and photometric stellar luminosity functions different ?}",
  journal = {\apj},
   eprint = {astro-ph/9505128},
     year = 1995,
    month = nov,
   volume = 453,
    pages = {350},
      doi = {10.1086/176394},
   adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...453..350K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{chabrier03,
   author = {{Chabrier}, G.},
    title = "{Galactic Stellar and Substellar Initial Mass Function}",
  journal = {\pasp},
   eprint = {astro-ph/0304382},
 keywords = {Galaxies: Luminosity Function, Mass Function, Invited Reviews},
     year = 2003,
    month = jul,
   volume = 115,
    pages = {763-795},
      doi = {10.1086/376392},
   adsurl = {http://adsabs.harvard.edu/abs/2003PASP..115..763C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{mckee07,
   author = {{McKee}, C.~F. and {Ostriker}, E.~C.},
    title = "{Theory of Star Formation}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {0707.3514},
     year = 2007,
    month = sep,
   volume = 45,
    pages = {565-687},
      doi = {10.1146/annurev.astro.45.051806.110602},
   adsurl = {http://adsabs.harvard.edu/abs/2007ARA%26A..45..565M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{zoccali03,
   author = {{Zoccali}, M. and {Renzini}, A. and {Ortolani}, S. and {Greggio}, L. and 
	{Saviane}, I. and {Cassisi}, S. and {Rejkuba}, M. and {Barbuy}, B. and 
	{Rich}, R.~M. and {Bica}, E.},
    title = "{Age and metallicity distribution of the Galactic bulge  from extensive optical and near-IR stellar photometry}",
  journal = {\aap},
   eprint = {astro-ph/0210660},
 keywords = {Galaxy: bulge, stars: Hertzsprung-Russell (H-R) and C-M diagrams, stars: luminosity function, mass function},
     year = 2003,
    month = mar,
   volume = 399,
    pages = {931-956},
      doi = {10.1051/0004-6361:20021604},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...399..931Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{zoccali00,
   author = {{Zoccali}, M. and {Cassisi}, S. and {Frogel}, J.~A. and {Gould}, A. and 
	{Ortolani}, S. and {Renzini}, A. and {Rich}, R.~M. and {Stephens}, A.~W.
	},
    title = "{The Initial Mass Function of the Galactic Bulge down to \~{}0.15 M$_{solar}$}",
  journal = {\apj},
   eprint = {astro-ph/9906452},
 keywords = {INFRARED: STARS, STARS: LUMINOSITY FUNCTION, MASS FUNCTION, STARS: STATISTICS},
     year = 2000,
    month = feb,
   volume = 530,
    pages = {418-428},
      doi = {10.1086/308359},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...530..418Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bressan12,
   author = {{Bressan}, A. and {Marigo}, P. and {Girardi}, L. and {Salasnich}, B. and 
	{Dal Cero}, C. and {Rubele}, S. and {Nanni}, A.},
    title = "{PARSEC: stellar tracks and isochrones with the PAdova and TRieste Stellar Evolution Code}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1208.4498},
 primaryClass = "astro-ph.SR",
 keywords = {stars: evolution, Hertzsprung{\dash}Russell and colour magnitude diagrams, stars: interiors, stars: low-mass},
     year = 2012,
    month = nov,
   volume = 427,
    pages = {127-145},
      doi = {10.1111/j.1365-2966.2012.21948.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.427..127B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{cignoni13,
   author = {{Cignoni}, M. and {Cole}, A.~A. and {Tosi}, M. and {Gallagher}, J.~S. and 
	{Sabbi}, E. and {Anderson}, J. and {Grebel}, E.~K. and {Nota}, A.
	},
    title = "{Mean Age Gradient and Asymmetry in the Star Formation History of the Small Magellanic Cloud}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1308.1409},
 primaryClass = "astro-ph.GA",
 keywords = {galaxies: dwarf, galaxies: evolution, galaxies: formation, galaxies: individual: Small Magellanic Cloud, galaxies: star formation, galaxies: stellar content, galaxies: structure, Hertzsprung-Russell and C-M diagrams, Magellanic Clouds, stars: statistics },
     year = 2013,
    month = oct,
   volume = 775,
      eid = {83},
    pages = {83},
      doi = {10.1088/0004-637X/775/2/83},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...775...83C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{fukugita98,
   author = {{Fukugita}, M. and {Hogan}, C.~J. and {Peebles}, P.~J.~E.},
    title = "{The Cosmic Baryon Budget}",
  journal = {\apj},
   eprint = {astro-ph/9712020},
 keywords = {COSMOLOGY: OBSERVATIONS, ELEMENTARY PARTICLES, GALAXIES: FUNDAMENTAL PARAMETERS, Cosmology: Observations, Elementary Particles, Galaxies: Fundamental Parameters},
     year = 1998,
    month = aug,
   volume = 503,
    pages = {518-530},
      doi = {10.1086/306025},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...503..518F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{calchi08,
   author = {{Calchi Novati}, S. and {de Luca}, F. and {Jetzer}, P. and {Mancini}, L. and 
	{Scarpetta}, G.},
    title = "{Microlensing constraints on the Galactic bulge initial mass function}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0711.3758},
 keywords = {gravitational lensing, Galaxy: bulge, Galaxy: stellar contents},
     year = 2008,
    month = mar,
   volume = 480,
    pages = {723-733},
      doi = {10.1051/0004-6361:20078439},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...480..723C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{holtz98,
   author = {{Holtzman}, J.~A. and {Watson}, A.~M. and {Baum}, W.~A. and 
	{Grillmair}, C.~J. and {Groth}, E.~J. and {Light}, R.~M. and 
	{Lynds}, R. and {O'Neil}, Jr., E.~J.},
    title = "{The Luminosity Function and Initial Mass Function in the Galactic Bulge}",
  journal = {\aj},
   eprint = {astro-ph/9801321},
 keywords = {GALAXIES: STELLAR CONTENT, STARS: LUMINOSITY FUNCTION, MASS FUNCTION},
     year = 1998,
    month = may,
   volume = 115,
    pages = {1946-1957},
      doi = {10.1086/300336},
   adsurl = {http://adsabs.harvard.edu/abs/1998AJ....115.1946H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{calamida2014b,
   author = {{Calamida}, A. and {Sahu}, K.~C. and {Anderson}, J. and {Casertano}, S. and 
	{Cassisi}, S. and {Salaris}, M. and {Brown}, T. and {Sokol}, J. and 
	{Bond}, H.~E. and {Ferraro}, I. and {Ferguson}, H. and {Livio}, M. and 
	{Valenti}, J. and {Buonanno}, R. and {Clarkson}, W. and {Pietrinferni}, A.
	},
    title = "{First Detection of the White Dwarf Cooling Sequence of the Galactic Bulge}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1406.6451},
 primaryClass = "astro-ph.SR",
 keywords = {stars: abundances, stars: evolution},
     year = 2014,
    month = aug,
   volume = 790,
      eid = {164},
    pages = {164},
      doi = {10.1088/0004-637X/790/2/164},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...790..164C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{taylor01,
   author = {{Taylor}, J.~M. and {Grindlay}, J.~E. and {Edmonds}, P.~D. and 
	{Cool}, A.~M.},
    title = "{Helium White Dwarfs and BY Draconis Binaries in the Globular Cluster NGC 6397}",
  journal = {\apjl},
 keywords = {Stars: Binaries: Close, Stars: Binaries: Eclipsing, Galaxy: Globular Clusters: General, Galaxy: Globular Clusters: Individual: NGC Number: NGC 6397, Stars: Individual: Constellation Name: BY Draconis, Stars: Neutron, Stars: Rotation, Stellar Dynamics, Stars: White Dwarfs},
     year = 2001,
    month = jun,
   volume = 553,
    pages = {L169-L172},
      doi = {10.1086/320676},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...553L.169T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{richer08,
   author = {{Richer}, H.~B. and {Dotter}, A. and {Hurley}, J. and {Anderson}, J. and 
	{King}, I. and {Davis}, S. and {Fahlman}, G.~G. and {Hansen}, B.~M.~S. and 
	{Kalirai}, J. and {Paust}, N. and {Rich}, R.~M. and {Shara}, M.~M.
	},
    title = "{Deep Advanced Camera for Surveys Imaging in the Globular Cluster NGC 6397: the Cluster Color-Magnitude Diagram and Luminosity Function}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {0708.4030},
 keywords = {Galaxy: halo, globular clusters: individual: NGC 6397, stars: low-mass, brown dwarfs, stars: luminosity function, mass function, stars: Population II, white dwarfs},
     year = 2008,
    month = jun,
   volume = 135,
    pages = {2141-2154},
      doi = {10.1088/0004-6256/135/6/2141},
   adsurl = {http://adsabs.harvard.edu/abs/2008AJ....135.2141R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{rebassa07,
   author = {{Rebassa-Mansergas}, A. and {G{\"a}nsicke}, B.~T. and {Rodr{\'{\i}}guez-Gil}, P. and 
	{Schreiber}, M.~R. and {Koester}, D.},
    title = "{Post-common-envelope binaries from SDSS - I. 101 white dwarf main-sequence binaries with multiple Sloan Digital Sky Survey spectroscopy}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0707.4107},
 keywords = {accretion, accretion discs, binaries: close, novae, cataclysmic variables},
     year = 2007,
    month = dec,
   volume = 382,
    pages = {1377-1393},
      doi = {10.1111/j.1365-2966.2007.12288.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.382.1377R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{wacther03,
   author = {{Wachter}, S. and {Hoard}, D.~W. and {Hansen}, K.~H. and {Wilcox}, R.~E. and 
	{Taylor}, H.~M. and {Finkelstein}, S.~L.},
    title = "{Cool Companions to White Dwarfs from the Two Micron All-Sky Survey Second Incremental Data Release}",
  journal = {\apj},
   eprint = {astro-ph/0212174},
 keywords = {Stars: Binaries: General, Infrared: Stars, Stars: Fundamental Parameters, Surveys, Stars: White Dwarfs},
     year = 2003,
    month = apr,
   volume = 586,
    pages = {1356-1363},
      doi = {10.1086/367821},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...586.1356W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{brown10,
   author = {{Brown}, T.~M. and {Sahu}, K. and {Anderson}, J. and {Tumlinson}, J. and 
	{Valenti}, J.~A. and {Smith}, E. and {Jeffery}, E.~J. and {Renzini}, A. and 
	{Zoccali}, M. and {Ferguson}, H.~C. and {VandenBerg}, D.~A. and 
	{Bond}, H.~E. and {Casertano}, S. and {Valenti}, E. and {Minniti}, D. and 
	{Livio}, M. and {Panagia}, N.},
    title = "{The WFC3 Galactic Bulge Treasury Program: Metallicity Estimates for the Stellar Population and Exoplanet Hosts}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1011.0457},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: bulge, Galaxy: formation, Galaxy: stellar content, planetary systems, stars: low-mass, techniques: photometric},
     year = 2010,
    month = dec,
   volume = 725,
    pages = {L19-L23},
      doi = {10.1088/2041-8205/725/1/L19},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...725L..19B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{aung07,
   author = {{Aungwerojwit}, A. and {G{\"a}nsicke}, B.~T. and {Rodr{\'{\i}}guez-Gil}, P. and 
	{Hagen}, H.-J. and {Giannakis}, O. and {Papadimitriou}, C. and 
	{Allende Prieto}, C. and {Engels}, D.},
    title = "{HS 1857+5144: a hot and young pre-cataclysmic variable}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0704.1780},
 keywords = {stars: binaries: close, stars: individual: HS 1857+5144},
     year = 2007,
    month = jul,
   volume = 469,
    pages = {297-305},
      doi = {10.1051/0004-6361:20077276},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...469..297A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{weissferguson09,
   author = {{Weiss}, A. and {Ferguson}, J.~W.},
    title = "{New asymptotic giant branch models for a range of metallicities}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0903.2155},
 primaryClass = "astro-ph.SR",
 keywords = {stars: evolution, stars: AGB and post-AGB, stars: interiors},
     year = 2009,
    month = dec,
   volume = 508,
    pages = {1343-1358},
      doi = {10.1051/0004-6361/200912043},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...508.1343W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{saito11,
   author = {{Saito}, R.~K. and {Zoccali}, M. and {McWilliam}, A. and {Minniti}, D. and 
	{Gonzalez}, O.~A. and {Hill}, V.},
    title = "{Mapping the X-shaped Milky Way Bulge}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1107.5360},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: bulge, Galaxy: structure, stars: distances, stars: late-type},
     year = 2011,
    month = sep,
   volume = 142,
      eid = {76},
    pages = {76},
      doi = {10.1088/0004-6256/142/3/76},
   adsurl = {http://adsabs.harvard.edu/abs/2011AJ....142...76S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{saito12,
   author = {{Saito}, R.~K. and {Hempel}, M. and {Minniti}, D. and {Lucas}, P.~W. and 
	{Rejkuba}, M. and {Toledo}, I. and {Gonzalez}, O.~A. and {Alonso-Garc{\'{\i}}a}, J. and 
	{Irwin}, M.~J. and {Gonzalez-Solares}, E. and {Hodgkin}, S.~T. and 
	{Lewis}, J.~R. and {Cross}, N. and {Ivanov}, V.~D. and {Kerins}, E. and 
	{Emerson}, J.~P. and {Soto}, M. and {Am{\^o}res}, E.~B. and 
	{Gurovich}, S. and {D{\'e}k{\'a}ny}, I. and {Angeloni}, R. and 
	{Beamin}, J.~C. and {Catelan}, M. and {Padilla}, N. and {Zoccali}, M. and 
	{Pietrukowicz}, P. and {Moni Bidin}, C. and {Mauro}, F. and 
	{Geisler}, D. and {Folkes}, S.~L. and {Sale}, S.~E. and {Borissova}, J. and 
	{Kurtev}, R. and {Ahumada}, A.~V. and {Alonso}, M.~V. and {Adamson}, A. and 
	{Arias}, J.~I. and {Bandyopadhyay}, R.~M. and {Barb{\'a}}, R.~H. and 
	{Barbuy}, B. and {Baume}, G.~L. and {Bedin}, L.~R. and {Bellini}, A. and 
	{Benjamin}, R. and {Bica}, E. and {Bonatto}, C. and {Bronfman}, L. and 
	{Carraro}, G. and {Chen{\`e}}, A.~N. and {Clari{\'a}}, J.~J. and 
	{Clarke}, J.~R.~A. and {Contreras}, C. and {Corvill{\'o}n}, A. and 
	{de Grijs}, R. and {Dias}, B. and {Drew}, J.~E. and {Fari{\~n}a}, C. and 
	{Feinstein}, C. and {Fern{\'a}ndez-Laj{\'u}s}, E. and {Gamen}, R.~C. and 
	{Gieren}, W. and {Goldman}, B. and {Gonz{\'a}lez-Fern{\'a}ndez}, C. and 
	{Grand}, R.~J.~J. and {Gunthardt}, G. and {Hambly}, N.~C. and 
	{Hanson}, M.~M. and {He{\l}miniak}, K.~G. and {Hoare}, M.~G. and 
	{Huckvale}, L. and {Jord{\'a}n}, A. and {Kinemuchi}, K. and 
	{Longmore}, A. and {L{\'o}pez-Corredoira}, M. and {Maccarone}, T. and 
	{Majaess}, D. and {Mart{\'{\i}}n}, E.~L. and {Masetti}, N. and 
	{Mennickent}, R.~E. and {Mirabel}, I.~F. and {Monaco}, L. and 
	{Morelli}, L. and {Motta}, V. and {Palma}, T. and {Parisi}, M.~C. and 
	{Parker}, Q. and {Pe{\~n}aloza}, F. and {Pietrzy{\'n}ski}, G. and 
	{Pignata}, G. and {Popescu}, B. and {Read}, M.~A. and {Rojas}, A. and 
	{Roman-Lopes}, A. and {Ruiz}, M.~T. and {Saviane}, I. and {Schreiber}, M.~R. and 
	{Schr{\"o}der}, A.~C. and {Sharma}, S. and {Smith}, M.~D. and 
	{Sodr{\'e}}, L. and {Stead}, J. and {Stephens}, A.~W. and {Tamura}, M. and 
	{Tappert}, C. and {Thompson}, M.~A. and {Valenti}, E. and {Vanzi}, L. and 
	{Walton}, N.~A. and {Weidmann}, W. and {Zijlstra}, A.},
    title = "{VVV DR1: The first data release of the Milky Way bulge and southern plane from the near-infrared ESO public survey VISTA variables in the V{\'{\i}}a L{\'a}ctea}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1111.5511},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: bulge, Galaxy: disk, Galaxy: stellar content, stars:, abundances, infrared: stars, surveys},
     year = 2012,
    month = jan,
   volume = 537,
      eid = {A107},
    pages = {A107},
      doi = {10.1051/0004-6361/201118407},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...537A.107S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{iben97,
   author = {{Iben}, Jr., I. and {Tutukov}, A.~V. and {Yungelson}, L.~R.},
    title = "{Helium and Carbon-Oxygen White Dwarfs in Close Binaries}",
  journal = {\apj},
 keywords = {STARS: BINARIES: CLOSE, STARS: EVOLUTION, STARS: INTERIORS, STARS: WHITE DWARFS},
     year = 1997,
    month = jan,
   volume = 475,
    pages = {291},
      doi = {10.1086/303525},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...475..291I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{yungelson94,
   author = {{Yungelson}, L.~R. and {Livio}, M. and {Tutukov}, A.~V. and 
	{Saffer}, R.~A.},
    title = "{Are the observed frequencies of double degenerates and SN IA contradictory?}",
  journal = {\apj},
 keywords = {BINARY STARS, DEGENERATE MATTER, STAR FORMATION, SUPERNOVAE, WHITE DWARF STARS, ASTROPHYSICS, STELLAR EVOLUTION, STELLAR MASS},
     year = 1994,
    month = jan,
   volume = 420,
    pages = {336-340},
      doi = {10.1086/173563},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...420..336Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{darnley12,
   author = {{Darnley}, M.~J. and {Ribeiro}, V.~A.~R.~M. and {Bode}, M.~F. and 
	{Hounsell}, R.~A. and {Williams}, R.~P.},
    title = "{On the Progenitors of Galactic Novae}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1112.2589},
 primaryClass = "astro-ph.SR",
 keywords = {novae, cataclysmic variables},
     year = 2012,
    month = feb,
   volume = 746,
      eid = {61},
    pages = {61},
      doi = {10.1088/0004-637X/746/1/61},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...746...61D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bedin05a,
   author = {{Bedin}, L.~R. and {Cassisi}, S. and {Castelli}, F. and {Piotto}, G. and 
	{Anderson}, J. and {Salaris}, M. and {Momany}, Y. and {Pietrinferni}, A.
	},
    title = "{Transforming observational data and theoretical isochrones into the ACS/WFC Vega-mag system}",
  journal = {\mnras},
   eprint = {astro-ph/0412328},
 keywords = {techniques: photometric, Hertzsprung-Russell (HR) diagram, stars: imaging},
     year = 2005,
    month = mar,
   volume = 357,
    pages = {1038-1048},
      doi = {10.1111/j.1365-2966.2005.08735.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.357.1038B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{hauschildt99,
   author = {{Hauschildt}, P.~H. and {Allard}, F. and {Ferguson}, J. and 
	{Baron}, E. and {Alexander}, D.~R.},
    title = "{The NEXTGEN Model Atmosphere Grid. II. Spherically Symmetric Model Atmospheres for Giant Stars with Effective Temperatures between 3000 and 6800 K}",
  journal = {\apj},
   eprint = {astro-ph/9907194},
 keywords = {RADIATIVE TRANSFER, STARS: ATMOSPHERES, STARS: LATE-TYPE},
     year = 1999,
    month = nov,
   volume = 525,
    pages = {871-880},
      doi = {10.1086/307954},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...525..871H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{buonannoiannicola89,
   author = {{Buonanno}, R. and {Iannicola}, G.},
    title = "{Stellar photometry with big pixels}",
  journal = {\pasp},
 keywords = {IMAGE PROCESSING, PIXELS, STELLAR SPECTROPHOTOMETRY, CHARGE COUPLED DEVICES, INTEGRAL EQUATIONS, STAR DISTRIBUTION, STELLAR MAGNITUDE},
     year = 1989,
    month = mar,
   volume = 101,
    pages = {294-301},
      doi = {10.1086/132434},
   adsurl = {http://adsabs.harvard.edu/abs/1989PASP..101..294B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{kalirai09,
   author = {{Kalirai}, J.~S. and {Saul Davis}, D. and {Richer}, H.~B. and 
	{Bergeron}, P. and {Catelan}, M. and {Hansen}, B.~M.~S. and 
	{Rich}, R.~M.},
    title = "{The Masses of Population II White Dwarfs}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0909.2253},
 primaryClass = "astro-ph.SR",
 keywords = {globular clusters: individual: M4, stars: evolution, stars: mass loss, techniques: spectroscopic, white dwarfs},
     year = 2009,
    month = nov,
   volume = 705,
    pages = {408-425},
      doi = {10.1088/0004-637X/705/1/408},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...705..408K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{dantona10,
   author = {{D'Antona}, F. and {Caloi}, V. and {Ventura}, P.},
    title = "{The evolutionary status of the blue hook stars in {$\omega$} Centauri}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1003.2052},
 primaryClass = "astro-ph.GA",
 keywords = {stars: abundances, stars: horizontal branch, stars: subdwarfs, globular clusters: individual: Omega Cen},
     year = 2010,
    month = jul,
   volume = 405,
    pages = {2295-2301},
      doi = {10.1111/j.1365-2966.2010.16646.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.405.2295D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{salaris09,
   author = {{Salaris}, M. and {Serenelli}, A. and {Weiss}, A. and {Miller Bertolami}, M.
	},
    title = "{Semi-empirical White Dwarf Initial-Final Mass Relationships: A Thorough Analysis of Systematic Uncertainties Due to Stellar Evolution Models}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0807.3567},
 keywords = {stars: AGB and post-AGB, stars: evolution, stars: individual: Sirius, stars: mass loss, white dwarfs, open clusters and associations: individual: Pleiades Hyades Praesepe NGC 1039 NGC 2168 NGC 2099 NGC 2516 NGC 3532 NGC 6819 NGC 7789},
     year = 2009,
    month = feb,
   volume = 692,
    pages = {1013-1032},
      doi = {10.1088/0004-637X/692/2/1013},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...692.1013S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{pietrinferni04,
   author = {{Pietrinferni}, A. and {Cassisi}, S. and {Salaris}, M. and {Castelli}, F.
	},
    title = "{A Large Stellar Evolution Database for Population Synthesis Studies. I. Scaled Solar Models and Isochrones}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0405193},
 keywords = {Galaxies: Stellar Content, Galaxy: Disk, Galaxy: Open Clusters and Associations: General, Stars: Evolution, Stars: Horizontal-Branch},
     year = 2004,
    month = sep,
   volume = 612,
    pages = {168-190},
      doi = {10.1086/422498},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...612..168P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{bensby13,
   author = {{Bensby}, T. and {Yee}, J.~C. and {Feltzing}, S. and {Johnson}, J.~A. and 
	{Gould}, A. and {Cohen}, J.~G. and {Asplund}, M. and {Mel{\'e}ndez}, J. and 
	{Lucatello}, S. and {Han}, C. and {Thompson}, I. and {Gal-Yam}, A. and 
	{Udalski}, A. and {Bennett}, D.~P. and {Bond}, I.~A. and {Kohei}, W. and 
	{Sumi}, T. and {Suzuki}, D. and {Suzuki}, K. and {Takino}, S. and 
	{Tristram}, P. and {Yamai}, N. and {Yonehara}, A.},
    title = "{Chemical evolution of the Galactic bulge as traced by microlensed dwarf and subgiant stars. V. Evidence for a wide age distribution and a complex MDF}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1211.6848},
 primaryClass = "astro-ph.GA",
 keywords = {gravitational lensing: micro, Galaxy: bulge, Galaxy:, formation, Galaxy: evolution, stars: abundances},
     year = 2013,
    month = jan,
   volume = 549,
      eid = {A147},
    pages = {A147},
      doi = {10.1051/0004-6361/201220678},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...549A.147B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{ness13,
   author = {{Ness}, M. and {Freeman}, K. and {Athanassoula}, E. and {Wylie-de-Boer}, E. and 
	{Bland-Hawthorn}, J. and {Asplund}, M. and {Lewis}, G.~F. and 
	{Yong}, D. and {Lane}, R.~R. and {Kiss}, L.~L.},
    title = "{ARGOS - III. Stellar populations in the Galactic bulge of the Milky Way}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1212.1540},
 primaryClass = "astro-ph.GA",
 keywords = {stars: abundances, Galaxy: abundances, Galaxy: bulge, Galaxy: centre, Galaxy: evolution, Galaxy: formation},
     year = 2013,
    month = apr,
   volume = 430,
    pages = {836-857},
      doi = {10.1093/mnras/sts629},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.430..836N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{hill11,
   author = {{Hill}, V. and {Lecureur}, A. and {G{\'o}mez}, A. and {Zoccali}, M. and 
	{Schultheis}, M. and {Babusiaux}, C. and {Royer}, F. and {Barbuy}, B. and 
	{Arenou}, F. and {Minniti}, D. and {Ortolani}, S.},
    title = "{The metallicity distribution of bulge clump giants in Baade's window}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1107.5199},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: bulge, Galaxy: formation, Galaxy: abundances, stars: abundances, stars: atmospheres},
     year = 2011,
    month = oct,
   volume = 534,
      eid = {A80},
    pages = {A80},
      doi = {10.1051/0004-6361/200913757},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...534A..80H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{heber09,
   author = {{Heber}, U.},
    title = "{Hot Subdwarf Stars}",
  journal = {\araa},
     year = 2009,
    month = sep,
   volume = 47,
    pages = {211-251},
      doi = {10.1146/annurev-astro-082708-101836},
   adsurl = {http://adsabs.harvard.edu/abs/2009ARA%26A..47..211H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{kilic12,
   author = {{Kilic}, M. and {Brown}, W.~R. and {Allende Prieto}, C. and 
	{Kenyon}, S.~J. and {Heinke}, C.~O. and {Ag{\"u}eros}, M.~A. and 
	{Kleinman}, S.~J.},
    title = "{The ELM Survey. IV. 24 White Dwarf Merger Systems}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1204.0028},
 primaryClass = "astro-ph.GA",
 keywords = {binaries: close, Galaxy: stellar content, gravitational waves, supernovae: general, white dwarfs},
     year = 2012,
    month = jun,
   volume = 751,
      eid = {141},
    pages = {141},
      doi = {10.1088/0004-637X/751/2/141},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...751..141K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kilic07,
   author = {{Kilic}, M. and {Stanek}, K.~Z. and {Pinsonneault}, M.~H.},
    title = "{The Future Is Now: The Formation of Single Low-Mass White Dwarfs in the Solar Neighborhood}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0706.3045},
 keywords = {Stars: Low-Mass, Brown Dwarfs, Stars: White Dwarfs},
     year = 2007,
    month = dec,
   volume = 671,
    pages = {761-766},
      doi = {10.1086/522228},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...671..761K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{monibidin09,
   author = {{Moni Bidin}, C. and {Moehler}, S. and {Piotto}, G. and {Momany}, Y. and 
	{Recio-Blanco}, A.},
    title = "{A lack of close binaries among hot horizontal branch stars in globular clusters. M 80 and NGC 5986}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0903.2072},
 primaryClass = "astro-ph.GA",
 keywords = {stars: horizontal-branch, binaries: close, binaries: spectroscopic, stars: fundamental parameters, globular clusters: individual: <ASTROBJ>M 80</ASTROBJ>, globular clusters: individual: <ASTROBJ>NGC 5986</ASTROBJ>},
     year = 2009,
    month = may,
   volume = 498,
    pages = {737-751},
      doi = {10.1051/0004-6361/200810579},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...498..737M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{monibidin08,
   author = {{Moni Bidin}, C. and {Catelan}, M. and {Altmann}, M.},
    title = "{Is a binary fraction-age relation responsible for the lack of EHB binaries in globular clusters?}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0801.4795},
 keywords = {stars: horizontal-branch, binaries: close, binaries: spectroscopic, stars: subdwarfs, globular clusters: individual: <ASTROBJ>NGC 6752</ASTROBJ>},
     year = 2008,
    month = mar,
   volume = 480,
    pages = {L1-L4},
      doi = {10.1051/0004-6361:20078782},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...480L...1M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{maxted00,
   author = {{Maxted}, P.~F.~L. and {Marsh}, T.~R. and {Moran}, C.~K.~J.},
    title = "{Radial velocity measurements of white dwarfs}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0007129},
 keywords = {BINARIES: CLOSE, BINARIES: SPECTROSCOPIC, WHITE DWARFS},
     year = 2000,
    month = nov,
   volume = 319,
    pages = {305-317},
      doi = {10.1046/j.1365-8711.2000.03840.x},
   adsurl = {http://adsabs.harvard.edu/abs/2000MNRAS.319..305M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cassisi00,
   author = {{Cassisi}, S. and {Castellani}, V. and {Ciarcelluti}, P. and 
	{Piotto}, G. and {Zoccali}, M.},
    title = "{Galactic globular clusters as a test for very-low-mass stellar models}",
  journal = {\mnras},
   eprint = {astro-ph/0003003},
 keywords = {STARS: EVOLUTION, STARS: INTERIORS, GLOBULAR CLUSTERS: GENERAL},
     year = 2000,
    month = jul,
   volume = 315,
    pages = {679-688},
      doi = {10.1046/j.1365-8711.2000.03457.x},
   adsurl = {http://adsabs.harvard.edu/abs/2000MNRAS.315..679C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{cassisi03,
   author = {{Cassisi}, S. and {Schlattl}, H. and {Salaris}, M. and {Weiss}, A.
	},
    title = "{First Full Evolutionary Computation of the Helium Flash-induced Mixing in Population II Stars}",
  journal = {\apjl},
   eprint = {arXiv:astro-ph/0211498},
 keywords = {Stars: Abundances, Stars: Evolution, Stars: Horizontal-Branch, Stars: Late-Type},
     year = 2003,
    month = jan,
   volume = 582,
    pages = {L43-L46},
      doi = {10.1086/346200},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...582L..43C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{salaris10,
   author = {{Salaris}, M. and {Cassisi}, S. and {Pietrinferni}, A. and {Kowalski}, P.~M. and 
	{Isern}, J.},
    title = "{A Large Stellar Evolution Database for Population Synthesis Studies. VI. White Dwarf Cooling Sequences}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1005.1791},
 primaryClass = "astro-ph.SR",
 keywords = {Galaxy: disk, galaxies: stellar content, stars: evolution, stars: interiors, white dwarfs},
     year = 2010,
    month = jun,
   volume = 716,
    pages = {1241-1251},
      doi = {10.1088/0004-637X/716/2/1241},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...716.1241S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ferraro03,
   author = {{Ferraro}, F.~R. and {Possenti}, A. and {Sabbi}, E. and {D'Amico}, N.
	},
    title = "{The Helium White Dwarf Orbiting the Millisecond Pulsar in the Halo of the Globular Cluster NGC 6752}",
  journal = {\apjl},
   eprint = {arXiv:astro-ph/0309151},
 keywords = {Stars: Binaries: Close, Galaxy: Globular Clusters: Individual: NGC Number: NGC 6752, Stars: Pulsars: Individual: Alphanumeric: PSR J1911-5958A, Stars: Evolution},
     year = 2003,
    month = oct,
   volume = 596,
    pages = {L211-L214},
      doi = {10.1086/379536},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...596L.211F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{maxted01,
   author = {{Maxted}, P.~f.~L. and {Heber}, U. and {Marsh}, T.~R. and {North}, R.~C.
	},
    title = "{The binary fraction of extreme horizontal branch stars}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0103342},
 keywords = {binaries: close; binaries: spectroscopic; subdwarfs},
     year = 2001,
    month = oct,
   volume = 326,
    pages = {1391-1402},
      doi = {10.1111/j.1365-8711.2001.04714.x},
   adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.326.1391M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{bedin05b,
   author = {{Bedin}, L.~R. and {Salaris}, M. and {Piotto}, G. and {King}, I.~R. and 
	{Anderson}, J. and {Cassisi}, S. and {Momany}, Y.},
    title = "{The White Dwarf Cooling Sequence in NGC 6791}",
  journal = {\apjl},
   eprint = {arXiv:astro-ph/0503397},
 keywords = {Galaxy: Open Clusters and Associations: Individual: NGC Number: NGC 6791, Stars: White Dwarfs},
     year = 2005,
    month = may,
   volume = 624,
    pages = {L45-L48},
      doi = {10.1086/430310},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...624L..45B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{monelli05,
   author = {{Monelli}, M. and {Corsi}, C.~E. and {Castellani}, V. and {Ferraro}, I. and 
	{Iannicola}, G. and {Prada Moroni}, P.~G. and {Bono}, G. and 
	{Buonanno}, R. and {Calamida}, A. and {Freyhammer}, L.~M. and 
	{Pulone}, L. and {Stetson}, P.~B.},
    title = "{The Discovery of More than 2000 White Dwarfs in the Globular Cluster {$\omega$} Centauri}",
  journal = {\apjl},
   eprint = {arXiv:astro-ph/0501633},
 keywords = {Galaxy: Globular Clusters: General, Galaxy: Globular Clusters: Individual: Name: {$\omega$} Centauri},
     year = 2005,
    month = mar,
   volume = 621,
    pages = {L117-L120},
      doi = {10.1086/429255},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...621L.117M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{maxted02,
   author = {{Maxted}, P.~F.~L. and {Marsh}, T.~R. and {Heber}, U. and {Morales-Rueda}, L. and 
	{North}, R.~C. and {Lawson}, W.~A.},
    title = "{Photometry of four binary subdwarf B stars and the nature of their unseen companion stars}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0202177},
 keywords = {binaries: close, stars: horizontal branch, stars: individual: Feige 11, stars: individual: Ton 245, stars: individual: PG1017-086  stars: individual: PG1432+159},
     year = 2002,
    month = jun,
   volume = 333,
    pages = {231-240},
      doi = {10.1046/j.1365-8711.2002.05406.x},
   adsurl = {http://adsabs.harvard.edu/abs/2002MNRAS.333..231M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{marsh95,
   author = {{Marsh}, T.~R. and {Dhillon}, V.~S. and {Duck}, S.~R.},
    title = "{Low-Mass White Dwarfs Need Friends - Five New Double-Degenerate Close Binary Stars}",
  journal = {\mnras},
 keywords = {binaries: close - binaries: spectroscopic - white dwarfs},
     year = 1995,
    month = aug,
   volume = 275,
    pages = {828},
   adsurl = {http://adsabs.harvard.edu/abs/1995MNRAS.275..828M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{han02,
   author = {{Han}, Z. and {Podsiadlowski}, P. and {Maxted}, P.~F.~L. and 
	{Marsh}, T.~R. and {Ivanova}, N.},
    title = "{The origin of subdwarf B stars - I. The formation channels}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0206130},
 keywords = {methods: numerical, binaries: close, stars: formation, subdwarfs, white dwarfs},
     year = 2002,
    month = oct,
   volume = 336,
    pages = {449-466},
      doi = {10.1046/j.1365-8711.2002.05752.x},
   adsurl = {http://adsabs.harvard.edu/abs/2002MNRAS.336..449H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{kepler07,
   author = {{Kepler}, S.~O. and {Kleinman}, S.~J. and {Nitta}, A. and {Koester}, D. and 
	{Castanheira}, B.~G. and {Giovannini}, O. and {Costa}, A.~F.~M. and 
	{Althaus}, L.},
    title = "{White dwarf mass distribution in the SDSS}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0612277},
 keywords = {white dwarfs},
     year = 2007,
    month = mar,
   volume = 375,
    pages = {1315-1324},
      doi = {10.1111/j.1365-2966.2006.11388.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.375.1315K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{rebassa11,
   author = {{Rebassa-Mansergas}, A. and {Nebot G{\'o}mez-Mor{\'a}n}, A. and 
	{Schreiber}, M.~R. and {Girven}, J. and {G{\"a}nsicke}, B.~T.
	},
    title = "{Post-common envelope binaries from SDSS-X: the origin of low-mass white dwarfs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1012.3089},
 primaryClass = "astro-ph.SR",
 keywords = {binaries: close, binaries: spectroscopic, stars: evolution, white dwarfs},
     year = 2011,
    month = may,
   volume = 413,
    pages = {1121-1131},
      doi = {10.1111/j.1365-2966.2011.18200.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.413.1121R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{koester09,
   author = {{Koester}, D. and {Voss}, B. and {Napiwotzki}, R. and {Christlieb}, N. and 
	{Homeier}, D. and {Lisker}, T. and {Reimers}, D. and {Heber}, U.
	},
    title = "{High-resolution UVES/VLT spectra of white dwarfs observed for the ESO SN Ia Progenitor Survey. III. DA white dwarfs}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0908.2322},
 primaryClass = "astro-ph.SR",
 keywords = {stars: white dwarfs},
     year = 2009,
    month = oct,
   volume = 505,
    pages = {441-462},
      doi = {10.1051/0004-6361/200912531},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...505..441K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{eisenstein06,
   author = {{Eisenstein}, D.~J. and {Liebert}, J. and {Harris}, H.~C. and 
	{Kleinman}, S.~J. and {Nitta}, A. and {Silvestri}, N. and {Anderson}, S.~A. and 
	{Barentine}, J.~C. and {Brewington}, H.~J. and {Brinkmann}, J. and 
	{Harvanek}, M. and {Krzesi{\'n}ski}, J. and {Neilsen}, Jr., E.~H. and 
	{Long}, D. and {Schneider}, D.~P. and {Snedden}, S.~A.},
    title = "{A Catalog of Spectroscopically Confirmed White Dwarfs from the Sloan Digital Sky Survey Data Release 4}",
  journal = {\apjs},
   eprint = {arXiv:astro-ph/0606700},
 keywords = {Catalogs, Stars: Subdwarfs, Stars: White Dwarfs},
     year = 2006,
    month = nov,
   volume = 167,
    pages = {40-58},
      doi = {10.1086/507110},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJS..167...40E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kleinman13,
   author = {{Kleinman}, S.~J. and {Kepler}, S.~O. and {Koester}, D. and 
	{Pelisoli}, I. and {Pe{\c c}anha}, V. and {Nitta}, A. and {Costa}, J.~E.~S. and 
	{Krzesinski}, J. and {Dufour}, P. and {Lachapelle}, F.-R. and 
	{Bergeron}, P. and {Yip}, C.-W. and {Harris}, H.~C. and {Eisenstein}, D.~J. and 
	{Althaus}, L. and {C{\'o}rsico}, A.},
    title = "{SDSS DR7 White Dwarf Catalog}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1212.1222},
 primaryClass = "astro-ph.SR",
 keywords = {catalogs, magnetic fields, stars: luminosity function, mass function, surveys, white dwarfs },
     year = 2013,
    month = jan,
   volume = 204,
      eid = {5},
    pages = {5},
      doi = {10.1088/0067-0049/204/1/5},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJS..204....5K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bedin08,
   author = {{Bedin}, L.~R. and {Salaris}, M. and {Piotto}, G. and {Cassisi}, S. and 
	{Milone}, A.~P. and {Anderson}, J. and {King}, I.~R.},
    title = "{The Puzzling White Dwarf Cooling Sequence in NGC 6791: A Simple Solution}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0804.1792},
 keywords = {Galaxy: Open Clusters and Associations: Individual: NGC Number: NGC 6791, Stars: White Dwarfs},
     year = 2008,
    month = may,
   volume = 679,
    pages = {L29-L32},
      doi = {10.1086/589151},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...679L..29B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ibentutukov85,
   author = {{Iben}, Jr., I. and {Tutukov}, A.~V.},
    title = "{On the evolution of close binaries with components of initial mass between 3 solar masses and 12 solar masses}",
  journal = {\apjs},
 keywords = {BINARY STARS, COMPUTATIONAL ASTROPHYSICS, STELLAR EVOLUTION, STELLAR MASS EJECTION, WHITE DWARF STARS, ABUNDANCE, HERTZSPRUNG-RUSSELL DIAGRAM, ORBITAL ELEMENTS, ROCHE LIMIT, STELLAR CORES, STELLAR ENVELOPES, STELLAR MASS ACCRETION, STELLAR MODELS, STELLAR STRUCTURE, STELLAR TEMPERATURE},
     year = 1985,
    month = aug,
   volume = 58,
    pages = {661-710},
      doi = {10.1086/191054},
   adsurl = {http://adsabs.harvard.edu/abs/1985ApJS...58..661I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pradamoroni09,
   author = {{Prada Moroni}, P.~G. and {Straniero}, O.},
    title = "{Very low-mass white dwarfs with a C-O core}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0909.2742},
 primaryClass = "astro-ph.SR",
 keywords = {stars: evolution, stars: white dwarfs, stars: horizontal-branch, stars: interiors, stars: oscillations},
     year = 2009,
    month = dec,
   volume = 507,
    pages = {1575-1583},
      doi = {10.1051/0004-6361/200912847},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...507.1575P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{althaus09,
   author = {{Althaus}, L.~G. and {Panei}, J.~A. and {Romero}, A.~D. and 
	{Rohrmann}, R.~D. and {C{\'o}rsico}, A.~H. and {Garc{\'{\i}}a-Berro}, E. and 
	{Miller Bertolami}, M.~M.},
    title = "{Evolution and colors of helium-core white dwarf stars with high-metallicity progenitors}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0905.1939},
 primaryClass = "astro-ph.SR",
 keywords = {stars: evolution, stars: white dwarfs, diffusion, galaxies: clusters: general},
     year = 2009,
    month = jul,
   volume = 502,
    pages = {207-216},
      doi = {10.1051/0004-6361/200911640},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...502..207A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{edmonds01,
   author = {{Edmonds}, P.~D. and {Gilliland}, R.~L. and {Heinke}, C.~O. and 
	{Grindlay}, J.~E. and {Camilo}, F.},
    title = "{Optical Detection of a Variable Millisecond Pulsar Companion in 47 Tucanae}",
  journal = {\apjl},
   eprint = {arXiv:astro-ph/0107096},
 keywords = {Stars: Binaries: General, Galaxy: Globular Clusters: Individual: Name: 47 Tucanae, Stars: Pulsars: General, pulsars: individual (PSR J0024-7203U)},
     year = 2001,
    month = aug,
   volume = 557,
    pages = {L57-L60},
      doi = {10.1086/323122},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...557L..57E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{freeman13,
   author = {{Freeman}, K. and {Ness}, M. and {Wylie-de-Boer}, E. and {Athanassoula}, E. and 
	{Bland-Hawthorn}, J. and {Asplund}, M. and {Lewis}, G. and {Yong}, D. and 
	{Lane}, R. and {Kiss}, L. and {Ibata}, R.},
    title = "{ARGOS - II. The Galactic bulge survey}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1212.1541},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: bulge, Galaxy: evolution, Galaxy: formation, Galaxy: kinematics and dynamics, stars: abundances},
     year = 2013,
    month = feb,
   volume = 428,
    pages = {3660-3670},
      doi = {10.1093/mnras/sts305},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.428.3660F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{brocato99,
   author = {{Brocato}, E. and {Castellani}, V. and {Romaniello}, M.},
    title = "{A theoretical exploratory investigation on cluster white dwarfs}",
  journal = {\aap},
 keywords = {STARS: EVOLUTION, STARS: LUMINOSITY FUNCTION, MASS FUNCTION, STARS: WHITE DWARFS, GALAXY: GLOBULAR CLUSTERS: GENERAL, GALAXY: OPEN CLUSTERS AND ASSOCIATIONS: GENERAL},
     year = 1999,
    month = may,
   volume = 345,
    pages = {499-504},
   adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...345..499B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{foley10,
   author = {{Foley}, R.~J. and {Brown}, P.~J. and {Rest}, A. and {Challis}, P.~J. and 
	{Kirshner}, R.~P. and {Wood-Vasey}, W.~M.},
    title = "{Early- and Late-Time Observations of SN 2008ha: Additional Constraints for the Progenitor and Explosion}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0912.0732},
 primaryClass = "astro-ph.SR",
 keywords = {supernovae: general, supernovae: individual: SN 2008ha},
     year = 2010,
    month = jan,
   volume = 708,
    pages = {L61-L65},
      doi = {10.1088/2041-8205/708/1/L61},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...708L..61F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{cardelli89,
   author = {{Cardelli}, J.~A. and {Clayton}, G.~C. and {Mathis}, J.~S.},
    title = "{The relationship between infrared, optical, and ultraviolet extinction}",
  journal = {\apj},
 keywords = {INFRARED SPECTRA, INTERSTELLAR EXTINCTION, ULTRAVIOLET SPECTRA, VISIBLE SPECTRUM, COMPUTATIONAL ASTROPHYSICS, INTERSTELLAR MATTER, IUE},
     year = 1989,
    month = oct,
   volume = 345,
    pages = {245-256},
      doi = {10.1086/167900},
   adsurl = {http://adsabs.harvard.edu/abs/1989ApJ...345..245C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pietrinferni06,
   author = {{Pietrinferni}, A. and {Cassisi}, S. and {Salaris}, M. and {Castelli}, F.
	},
    title = "{A Large Stellar Evolution Database for Population Synthesis Studies. II. Stellar Models and Isochrones for an {$\alpha$}-enhanced Metal Distribution}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0603721},
 keywords = {Galaxies: Stellar Content, Galaxy: Globular Clusters: General, Stars: Evolution, Stars: Horizontal-Branch},
     year = 2006,
    month = may,
   volume = 642,
    pages = {797-812},
      doi = {10.1086/501344},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...642..797P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{dotter08,
   author = {{Dotter}, A. and {Chaboyer}, B. and {Jevremovi{\'c}}, D. and 
	{Kostov}, V. and {Baron}, E. and {Ferguson}, J.~W.},
    title = "{The Dartmouth Stellar Evolution Database}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {0804.4473},
 keywords = {Galaxy: Globular Clusters: General, Galaxy: Open Clusters and Associations: General, Stars: Evolution},
     year = 2008,
    month = sep,
   volume = 178,
    pages = {89-101},
      doi = {10.1086/589654},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJS..178...89D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{moehler2007,
   author = {{Moehler}, S. and {Dreizler}, S. and {Lanz}, T. and {Bono}, G. and 
	{Sweigart}, A.~V. and {Calamida}, A. and {Monelli}, M. and {Nonino}, M.
	},
    title = "{The hottest horizontal-branch stars in {$\omega$} Centauri. Late hot flasher vs. helium enrichment}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0709.2839},
 keywords = {stars: horizontal-branch, stars: evolution, techniques: spectroscopic, Galaxy: globular clusters: individual: {$\omega$} Centauri},
     year = 2007,
    month = nov,
   volume = 475,
    pages = {L5-L8},
      doi = {10.1051/0004-6361:20078509},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...475L...5M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{moehler2011,
   author = {{Moehler}, S. and {Dreizler}, S. and {Lanz}, T. and {Bono}, G. and 
	{Sweigart}, A.~V. and {Calamida}, A. and {Nonino}, M.},
    title = "{The hot horizontal-branch stars in {$\omega$} Centauri}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1009.3191},
 primaryClass = "astro-ph.SR",
 keywords = {stars: horizontal-branch, stars: evolution, techniques: spectroscopic, globular clusters: individual: NGC 5139},
     year = 2011,
    month = feb,
   volume = 526,
      eid = {A136},
    pages = {A136},
      doi = {10.1051/0004-6361/201015020},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...526A.136M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{castellani06,
   author = {{Castellani}, M. and {Castellani}, V. and {Prada Moroni}, P.~G.
	},
    title = "{Hot flashers and He dwarfs in galactic globulars}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0606026},
 keywords = {stars: evolution, stars: white dwarfs, stars: mass-loss},
     year = 2006,
    month = oct,
   volume = 457,
    pages = {569-573},
      doi = {10.1051/0004-6361:20064875},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...457..569C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{han08,
   author = {{Han}, Z.},
    title = "{A possible solution for the lack of EHB binaries in globular clusters}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0804.4535},
 keywords = {stars: horizontal-branch, binaries: close, stars: subdwarfs, globular clusters: general},
     year = 2008,
    month = jun,
   volume = 484,
    pages = {L31-L34},
      doi = {10.1051/0004-6361:200809614},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...484L..31H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lee05,
   author = {{Lee}, Y.-W. and {Joo}, S.-J. and {Han}, S.-I. and {Chung}, C. and 
	{Ree}, C.~H. and {Sohn}, Y.-J. and {Kim}, Y.-C. and {Yoon}, S.-J. and 
	{Yi}, S.~K. and {Demarque}, P.},
    title = "{Super-Helium-rich Populations and the Origin of Extreme Horizontal-Branch Stars in Globular Clusters}",
  journal = {\apjl},
   eprint = {arXiv:astro-ph/0501500},
 keywords = {Galaxy: Globular Clusters: Individual: Name: {$\omega$} Centauri, Galaxy: Globular Clusters: Individual: NGC Number: NGC 2808, Stars: Abundances, Stars: Evolution, Stars: Horizontal-Branch},
     year = 2005,
    month = mar,
   volume = 621,
    pages = {L57-L60},
      doi = {10.1086/428944},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...621L..57L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{castellani93,
   author = {{Castellani}, M. and {Castellani}, V.},
    title = "{Mass loss in globular cluster red giants - an evolutionary investigation}",
  journal = {\apj},
 keywords = {GLOBULAR CLUSTERS, RED GIANT STARS, STELLAR EVOLUTION, STELLAR MASS EJECTION, WHITE DWARF STARS, COOLING, STELLAR LUMINOSITY, STELLAR MODELS},
     year = 1993,
    month = apr,
   volume = 407,
    pages = {649-656},
      doi = {10.1086/172547},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...407..649C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{dcruz96,
   author = {{D'Cruz}, N.~L. and {Dorman}, B. and {Rood}, R.~T. and {O'Connell}, R.~W.
	},
    title = "{The Origin of Extreme Horizontal Branch Stars}",
  journal = {\apj},
 keywords = {GALAXIES: PHOTOMETRY, STARS: EVOLUTION, STARS: HORIZONTAL-BRANCH, STARS: INTERIORS, STARS: MASS LOSS, ULTRAVIOLET: GALAXIES},
     year = 1996,
    month = jul,
   volume = 466,
    pages = {359},
      doi = {10.1086/177515},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...466..359D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{kalirai07,
   author = {{Kalirai}, J.~S. and {Bergeron}, P. and {Hansen}, B.~M.~S. and 
	{Kelson}, D.~D. and {Reitzel}, D.~B. and {Rich}, R.~M. and {Richer}, H.~B.
	},
    title = "{Stellar Evolution in NGC 6791: Mass Loss on the Red Giant Branch and the Formation of Low-Mass White Dwarfs}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0705.0977},
 keywords = {Galaxy: Open Clusters and Associations: Individual: NGC Number: NGC 6791, Stars: Evolution, Stars: Mass Loss, Techniques: Photometric, Techniques: Spectroscopic, Stars: White Dwarfs},
     year = 2007,
    month = dec,
   volume = 671,
    pages = {748-760},
      doi = {10.1086/521922},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...671..748K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{strickler09,
   author = {{Strickler}, R.~R. and {Cool}, A.~M. and {Anderson}, J. and 
	{Cohn}, H.~N. and {Lugger}, P.~M. and {Serenelli}, A.~M.},
    title = "{Helium-core White Dwarfs in the Globular Cluster NGC 6397}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0904.3496},
 primaryClass = "astro-ph.GA",
 keywords = {binaries: general, globular clusters: individual: NGC 6397, stars: imaging, stars: Population II, stellar dynamics, white dwarfs},
     year = 2009,
    month = jul,
   volume = 699,
    pages = {40-55},
      doi = {10.1088/0004-637X/699/1/40},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...699...40S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{calamida2013a,
   author = {{Calamida}, A. and {Bono}, G. and {Lagioia}, E. P. and
   {Milone}, A. P. and {Fabrizio}, M. and {Saviane}, I. and {Moni Bidin}, C. and
   {Mauro}, F. and {Buonanno}, B.},
    title = "{Str\"omgren -- Near -- Infrared photometry of the Bulge. I. The globular cluster NGC~6528 and the Baade's Window.}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0712.0603},
 keywords = {Galaxy: Globular Clusters: General, Galaxy: Globular Clusters: Individual: Name: {$\omega$} Centauri},
     year = 2013,
    month = dec,
   volume = XX,
    pages = {XX},
      doi = {XX},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...673L..29C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{calamida2008,
   author = {{Calamida}, A. and {Corsi}, C.~E. and {Bono}, G. and {Stetson}, P.~B. and 
	{Prada Moroni}, P. and {Degl'Innocenti}, S. and {Ferraro}, I. and 
	{Iannicola}, G. and {Koester}, D. and {Pulone}, L. and {Monelli}, M. and 
	{Amico}, P. and {Buonanno}, R. and {Caputo}, F. and {D'Odorico}, S. and 
	{Freyhammer}, L.~M. and {Marchetti}, E. and {Nonino}, M. and 
	{Romaniello}, M.},
    title = "{On the White Dwarf Cooling Sequence of the Globular Cluster {$\omega$} Centauri}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0712.0603},
 keywords = {Galaxy: Globular Clusters: General, Galaxy: Globular Clusters: Individual: Name: {$\omega$} Centauri},
     year = 2008,
    month = jan,
   volume = 673,
    pages = {L29-L33},
      doi = {10.1086/527436},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...673L..29C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{bellini13,
   author = {{Bellini}, A. and {Anderson}, J. and {Salaris}, M. and {Cassisi}, S. and 
	{Bedin}, L.~R. and {Piotto}, G. and {Bergeron}, P.},
    title = "{A Double White-dwarf Cooling Sequence in {$\omega$} Centauri}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1305.0265},
 primaryClass = "astro-ph.GA",
 keywords = {globular clusters: individual: NGC 5139, Hertzsprung-Russell and C-M diagrams, stars: Population II, techniques: photometric, white dwarfs },
     year = 2013,
    month = jun,
   volume = 769,
      eid = {L32},
    pages = {L32},
      doi = {10.1088/2041-8205/769/2/L32},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...769L..32B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{clarkson11,
   author = {{Clarkson}, W.~I. and {Sahu}, K.~C. and {Anderson}, J. and {Rich}, R.~M. and 
	{Smith}, T.~E. and {Brown}, T.~M. and {Bond}, H.~E. and {Livio}, M. and 
	{Minniti}, D. and {Renzini}, A. and {Zoccali}, M.},
    title = "{The First Detection of Blue Straggler Stars in the Milky Way Bulge}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1105.4176},
 primaryClass = "astro-ph.GA",
 keywords = {binaries: close, blue stragglers, Galaxy: bulge, Galaxy: kinematics and dynamics, Galaxy: stellar content, Galaxy: structure},
     year = 2011,
    month = jul,
   volume = 735,
      eid = {37},
    pages = {37},
      doi = {10.1088/0004-637X/735/1/37},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...735...37C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{clarkson08,
   author = {{Clarkson}, W. and {Sahu}, K. and {Anderson}, J. and {Smith}, T.~E. and 
	{Brown}, T.~M. and {Rich}, R.~M. and {Casertano}, S. and {Bond}, H.~E. and 
	{Livio}, M. and {Minniti}, D. and {Panagia}, N. and {Renzini}, A. and 
	{Valenti}, J. and {Zoccali}, M.},
    title = "{Stellar Proper Motions in the Galactic Bulge from Deep Hubble Space Telescope ACS WFC Photometry}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0809.1682},
 keywords = {Galaxy: Bulge, Galaxy: Disk, Galaxy: Kinematics and Dynamics, Instrumentation: High Angular Resolution, Methods: Data Analysis, Techniques: Photometric},
     year = 2008,
    month = sep,
   volume = 684,
    pages = {1110-1142},
      doi = {10.1086/590378},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...684.1110C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{busso05,
   author = {{Busso}, G. and {Moehler}, S. and {Zoccali}, M. and {Heber}, U. and 
	{Yi}, S.~K.},
    title = "{Hot Subdwarfs in the Galactic Bulge}",
  journal = {\apjl},
   eprint = {arXiv:astro-ph/0509672},
 keywords = {Galaxy: Bulge, Stars: Horizontal-Branch, Stars: Subdwarfs, Ultraviolet: Galaxies},
     year = 2005,
    month = nov,
   volume = 633,
    pages = {L29-L32},
      doi = {10.1086/498212},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...633L..29B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{zoccali08,
   author = {{Zoccali}, M. and {Hill}, V. and {Lecureur}, A. and {Barbuy}, B. and 
	{Renzini}, A. and {Minniti}, D. and {G{\'o}mez}, A. and {Ortolani}, S.
	},
    title = "{The metal content of bulge field stars from FLAMES-GIRAFFE spectra. I. Stellar parameters and iron abundances}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0805.1218},
 keywords = {Galaxy: bulge, stars: abundances, stars: atmospheres},
     year = 2008,
    month = jul,
   volume = 486,
    pages = {177-189},
      doi = {10.1051/0004-6361:200809394},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...486..177Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{treu11,
   author = {{Treu}, T. and {Dutton}, A.~A. and {Auger}, M.~W. and {Marshall}, P.~J. and 
	{Bolton}, A.~S. and {Brewer}, B.~J. and {Koo}, D.~C. and {Koopmans}, L.~V.~E.
	},
    title = "{The SWELLS survey - I. A large spectroscopically selected sample of edge-on late-type lens galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1104.5663},
 primaryClass = "astro-ph.CO",
 keywords = {gravitational lensing: strong, galaxies: fundamental parameters, galaxies: haloes, galaxies: spiral, galaxies: structure},
     year = 2011,
    month = nov,
   volume = 417,
    pages = {1601-1620},
      doi = {10.1111/j.1365-2966.2011.19378.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.417.1601T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{oosterhoff,
   author = {{Oosterhoff}, P.~T. and {Ponsen}, J.},
    title = "{Variable stars in the galactic window Sagittarius I at {$\alpha$} = 17$^{h}$53$^{m}$, {$\delta$} = -29{\deg}02'}",
  journal = {Bulletin of the Astronomical Institutes of the Netherlands Supplement Series},
     year = 1968,
   volume = 3,
    pages = {79},
   adsurl = {http://adsabs.harvard.edu/abs/1968BANS....3...79O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{sahu06,
   author = {{Sahu}, K.~C. and {Casertano}, S. and {Bond}, H.~E. and {Valenti}, J. and 
	{Ed Smith}, T. and {Minniti}, D. and {Zoccali}, M. and {Livio}, M. and 
	{Panagia}, N. and {Piskunov}, N. and {Brown}, T.~M. and {Brown}, T. and 
	{Renzini}, A. and {Rich}, R.~M. and {Clarkson}, W. and {Lubow}, S.
	},
    title = "{Transiting extrasolar planetary candidates in the Galactic bulge}",
  journal = {\nat},
   eprint = {arXiv:astro-ph/0610098},
     year = 2006,
    month = oct,
   volume = 443,
    pages = {534-540},
      doi = {10.1038/nature05158},
   adsurl = {http://adsabs.harvard.edu/abs/2006Natur.443..534S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{hansliebert03,
   author = {{Hansen}, B.~M.~S. and {Liebert}, J.},
    title = "{Cool White Dwarfs}",
  journal = {\araa},
     year = 2003,
   volume = 41,
    pages = {465-515},
      doi = {10.1146/annurev.astro.41.081401.155117},
   adsurl = {http://adsabs.harvard.edu/abs/2003ARA%26A..41..465H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@TECHREPORT{anderson06,
   author = {{Anderson}, J. and {King}, I.~R.},
    title = "{PSFs, Photometry, and Astronomy for the ACS/WFC}",
 keywords = {Hubble Space Telescope, HST, Space Telescope Science Institute, Advanced Camera for Surveys, ACS, WFC, Wide Field Camera, PSF},
booktitle = {Instrument Science Report ACS 2006-01, 34 pages},
     year = 2006,
    month = feb,
    pages = {1},
   adsurl = {http://adsabs.harvard.edu/abs/2006acs..rept....1A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

